UniSparse: An Intermediate Language for General Sparse Format Customization

The ongoing trend of hardware specialization has led to a growing use of custom data formats when processing sparse workloads, which are typically memory-bound. These formats facilitate optimized software/hardware implementations by utilizing sparsity pattern- or target-aware data structures and layouts to enhance memory access latency and bandwidth utilization. However, existing sparse tensor programming models and compilers offer little or no support for productively customizing the sparse formats. Additionally, because these frameworks represent formats using a limited set of per-dimension attributes, they lack the flexibility to accommodate numerous new variations of custom sparse data structures and layouts. To overcome this deficiency, we propose UniSparse, an intermediate language that provides a unified abstraction for representing and customizing sparse formats. Unlike the existing attribute-based frameworks, UniSparse decouples the logical representation of the sparse tensor (i.e., the data structure) from its low-level memory layout, enabling the customization of both. As a result, a rich set of format customizations can be succinctly expressed in a small set of well-defined query, mutation, and layout primitives. We also develop a compiler leveraging the MLIR infrastructure, which supports adaptive customization of formats, and automatic code generation of format conversion and compute operations for heterogeneous architectures. We demonstrate the efficacy of our approach through experiments running commonly-used sparse linear algebra operations with specialized formats on multiple different hardware targets, including an Intel CPU, an NVIDIA GPU, an AMD Xilinx FPGA, and a simulated processing-in-memory (PIM) device.

==> figs-tabs/alg-emit-operator.tex <==
\begin{algorithm}
\caption{{Format Conversion}}
\label{alg:emit-op}
\KwIn{source format encoding \textbf{S}, target format encoding \textbf{T}, source format storage \textbf{S\_format}}
\KwOut{target format storage \textbf{T\_format}}
\begin{algorithmic}[1] % The number indicates the line numbering interval 
% \STATE s\_indirect\ = S.getIndirectFunc();\  t\_indirect = T.getIndirectFunc();
\STATE T\_format = S\_format; \COMMENT{in-place format storage conversion}
\IF{S.getIndexMap() != T.getIndexMap()}
    \IF{S.getIndexMap().getTile()}
        \STATE T\_format.convert(tile\_union); S.getIndexMap().update();
    \ENDIF
    \STATE affine\_trans = T.getIndexMap().to\_matrix() * S.getIndexMap().to\_matrix().inverse();
    \FOR{element\_trans in affine\_trans.decompose()}
    \ENDFOR
    \IF{T.getIndexMap().getTile()}
        \STATE T\_format.convert(tile\_split); S.getIndexMap().update();
    \ENDIF
    \STATE assert(!S.getIndirectFunc());
    \IF{T.getIndirectFunc()}
        \STATE T\_format.convert(\{rule\_5, rule\_6\});
    \ENDIF
    \STATE T\_format.sortIndices(); \COMMENT{sort indices in order}
\ENDIF
\WHILE{S.getTrimLevels() != T.getTrimLevels()}
    \STATE T\_format.convert(\{rule\_5, rule\_6\});  S.getTrimLevels().update();
\ENDWHILE
\WHILE{S.getMergeLevels() != T.getMergeLevels()}
    \STATE T\_format.convert(\{rule\_7\}); S.getMergeLevels().update();
\ENDWHILE
\STATE assert(!S.getLayout());
\IF{T.getLayout()}
    \STATE T\_format.pack()
    \STATE T\_format.partition()
\ENDIF
\RETURN T\_format
\end{algorithmic}
\end{algorithm}

% \STATE Sequence.push\_back(EmitDevectorize(src\_trims, dst\_trims));
% \STATE Sequence.push\_back(EmitReshape(src\_crd\_map, dst\_crd\_map));
% \STATE Sequence.push\_back(EmitArithmeticCoordinateMaps(src\_crd\_map, dst\_crd\_map));
% \STATE Sequence.push\_back(EmitStructureMutations(src\_trims, dst\_trims, src\_merges, dst\_merges));
% \STATE Sequence.push\_back(EmitVectorize(src\_trims, dst\_trims));
% \IF{D.parse\_IndirectCoordinateMap()}
%   \STATE Sequence.push\_back(EmitIndirectCoordinateMaps(src\_trims, dst\_trims));
% \ENDIF
% \IF{S != COO\_Encoding}
%   \STATE Sequence\_S = \textbf{Operator\_Emission}(COO\_Encoding, S);
%   \STATE Sequence\_D = \textbf{Operator\_Emission}(COO\_Encoding, D);
%   \STATE Shortcut\_Sequence = FindShortcut(Sequence\_S, Sequence\_D);
% \ENDIF
% \STATE Final\_Sequence = Compare(Sequence, Shortcut\_Sequence);
% \RETURN Final\_Sequence;

==> figs-tabs/fig-bdia-csr.tex <==
% \begin{figure*}[ht]
\begin{figure}[ht]
\centering
\includegraphics[scale=0.37]{images/spmv_dia_csr.pdf}
%\subfloat[SpMV kernel\label{subfig-1:spmv}]{%
%      \includegraphics[width=0.75\columnwidth]{images/spmv_dia_csr.pdf}
%    }
% \vfill
% \subfloat[PageRank application\label{subfig-2:pr}]{%
%       \centering
%       \includegraphics[width=0.68\columnwidth]{images/pr_dia-csr.pdf}
%     }
\vspace{-10pt}
\caption{Normalized run time of SpMV using the BDIA/CSR decomposed by \IRName vs. Intel MKL using the CSR on a 48-core CPU.}
\label{fig:BDIA_csr}
\vspace{-10pt}
\end{figure}
% \begin{subfigure}{0.49\textwidth}
%     \centering
%     \includegraphics[scale=0.4]{images/spmm_bell_coo.pdf}
%     \vspace{-10pt}
%     \caption{Normalized run time of cuSPARSE SpMM using the BELL/COO decomposed by \IRName vs. CSR on NVIDIA A6000. Datasets transformer-50 to 95 are pruned weight matrices of Transformer~\cite{sparse-weight} with sparsity ranging from 50\% to 95\%.}
%     \label{fig:bellpack}
    % \vspace{-5pt}
% \end{subfigure}
% \end{figure*}

==> figs-tabs/fig-code-example.tex <==
\begin{figure}[ht]
\begin{minipage}{\columnwidth}
% \centering
\begin{lstlisting}[
basicstyle={\scriptsize\ttfamily},
identifierstyle={\color{black}},
language={mlir},
numbersep=6pt,
numbers=left,
xleftmargin=2em, framexleftmargin=2em, aboveskip=1mm, belowskip=1mm,
escapeinside=**
]
// Format abstraction
#COO = #unisparse.encoding<{ 
        idx_map = #unisparse.map<(d0,d1)->(d0,d1)>, mutation = #unisparse.prim<trim(0,1)> }> *\label{spmv-format-abstraction}*
#CSR = #unisparse.encoding<{ 
        idx_map = #unisparse.map<(d0,d1)->(d0,d1)>, mutation = #unisparse.prim<merge(0), trim(1,1)> }>
#BDIA = #unisparse.encoding<{ 
        idx_map = #unisparse.map<(d0,d1)->(d0 div 50, d1-d0, d0 mod 50)>, mutation = #unisparse.prim<merge(0), trim(1,1)> }>
#COO_COO = #unisparse.hybrid<{ fmats = [#COO, #COO] }>
#BDIA_CSR = #unisparse.hybrid<{ fmats = [#BDIA, #CSR] }> *\label{spmv-format-abstraction-end}*
#sum = #unisparse.sum< groupBy (d0,d1) -> (d0 div 50, d1-d0), with val ne 0 -> 1 | otherwise -> 0 >

// Format pre-processing
%A1 = unisparse.decompose (%in_A, %thld) { query = #sum }: tensor<?x?xf32, #COO_COO> *\label{spmv-decompose}*
%A2 = unisparse.convert (%A1): tensor<?x?xf32, #BDIA_CSR> *\label{spmv-convert}*

// Compute operation
#spmv = { indexing_maps = [ *\label{spmv-signature}*
  affine_map<(d0,d1)->(d0,d1)>, // for argument %A21
  affine_map<(d0,d1)->(d1)>,     // for argument %in_X
  affine_map<(d0,d1)->(d0)>],  // for argument %out_Y
  iterator_types = ["parallel", "reduction"] }  *\label{spmv-signature-end}*
%0 = linalg.generic #spmv  *\label{spmv-linalg-generic}*
  ins(%A2, %in_X : tensor<?x?xf32, #BDIA_CSR>, tensor<?xf32>)
  outs(%out_Y: tensor<?xf32>) {
    ^bb0(%a: f32, %b: f32, %x: f32):
      %2 = arith.mulf %a, %b : f32 *\label{spmv-compute-start}*
      %3 = arith.addf %x, %2 : f32 *\label{spmv-compute-end}*
      linalg.yield %3 : f32
  } -> tensor<?xf32>  *\label{spmv-linalg-generic-end}*
\end{lstlisting}
\end{minipage}
% \begin{figure}
% \vspace{-8pt}
\caption{A \IRName program of the SpMV kernel with the hybrid BDIA/CSR format. The blocking size of the BDIA format is 50. File input operations are omitted. With the input tensor $A$ in COO format, the \lstinline{decompose} operation in Line \ref{spmv-decompose} divides the tensor into two sub-tensors adaptively by embedding a sparsity query primitive of \SumOp, and a \lstinline[morekeywords={convert}]{convert} operation in Line \ref{spmv-convert} translates the original format into a hybrid BDIA/CSR format. The SpMV kernel is specified using a \lstinline[alsoletter={\.},morekeywords={linalg\.generic}]{linalg\.generic} operation in Line~\ref{spmv-linalg-generic} - \ref{spmv-linalg-generic-end}.}
\label{fig-code}
\end{figure}

==> figs-tabs/fig-conversion-breakdown.tex <==
\begin{figure*}[ht]
\centering
% \subfloat[COO -> BDIA]{\>\includegraphics[scale=0.313]{images/BDIA-breakdown.pdf}\>%
% \label{BDIA-breakdown}}
% \subfloat[COO -> BELL]{\>\includegraphics[scale=0.313]{images/BELL-breakdown.pdf}\>%
% \label{BELL-breakdown}}
% \hfill
\subfloat[COO -> Serpens]{\>\includegraphics[scale=0.313]{images/serpens-breakdown.pdf}\>%
\label{serpens-breakdown}}
\subfloat[COO -> CISR-plus]{\>\includegraphics[scale=0.313]{images/CISRplus-breakdown.pdf}\>%
\label{CISR-plus-breakdown}}
\vspace{-8pt}
\caption{Breakdown of execution time (in \textit{seconds}) for each conversion operator, with the corresponding color coding shown in the legend in the center. For better readability, we use \textit{GM} as an abbreviation for Geomean results among all datasets, which applies to all illustrations below.}
\label{fig-breakdown}
\vspace{-8pt}
\end{figure*}

==> figs-tabs/fig-emitted-code.tex <==

\begin{figure}[ht]
\vspace{-5pt}
\begin{subfigure}[b]{0.326\linewidth}
\begin{lstlisting}[
basicstyle={\scriptsize\ttfamily},
identifierstyle={\color{black}},
tabsize=2,
numbers=left,
numbersep=8pt,
breaklines=true,
xleftmargin=2em, framexleftmargin=2em, aboveskip=1mm, belowskip=1mm,
escapeinside=<>
]
COO_structure
.tile_division(1, f)
.tile_division(0, f)
.shift(1, 2).sort(1) 
.merge(0)
.merge(1)
.fill(0)
.vectorize(2)
\end{lstlisting}
\caption{COO -> BCSR}
\label{fig-coo-bcsr-ir}
\end{subfigure}
\begin{subfigure}[b]{0.326\linewidth}
\begin{lstlisting}[
basicstyle={\scriptsize\ttfamily},
identifierstyle={\color{black}},
tabsize=2,
numbers=left,
numbersep=8pt,
breaklines=true,
xleftmargin=2em, framexleftmargin=2em, aboveskip=1mm, belowskip=1mm,
escapeinside=<>
]
COO_structure
.tile_division(1, f)
.tile_division(0, f)
.shift(1, 2).sort(1) 
.merge(0)
.merge(1)
.fill(0)
.vectorize(2)
.enumerate(1, 1, 0) 
.pad(2, 2) 
\end{lstlisting}
\caption{COO -> BELL}
\label{fig-coo-bell-ir}
\end{subfigure}
\begin{subfigure}[b]{0.326\linewidth}
\begin{lstlisting}[
basicstyle={\scriptsize\ttfamily},
identifierstyle={\color{black}},
tabsize=2,
numbers=left,
numbersep=8pt,
breaklines=true,
xleftmargin=2em, framexleftmargin=2em, aboveskip=1mm, belowskip=1mm,
escapeinside=<>
]
BCSR_structure
.enumerate(1, 1, 0)
.pad(2, 2)
\end{lstlisting}
\caption{BCSR -> BELL}
\label{fig-bcsr-bell-ir}
\end{subfigure}
\vspace{-8pt}
\caption{Examples of operator sequences generated during format conversion lowering in \IRName.}
\label{fig-example-ir}
\vspace{-8pt}
\end{figure}

==> figs-tabs/fig-index-tree.tex <==
\begin{figure*}[ht]
\centering
% \vspace{-7pt}
% \subfloat[Matrix $A$]{\includegraphics[scale=0.32]{images/matrix.pdf}%
% \label{matrix}}
% \hfil
\subfloat[COO or DOK]{\>\includegraphics[scale=0.32]{images/COO-DOK-tree.pdf}\>%
\label{COO-tree}}
\subfloat[CSR or LIL]{\>\includegraphics[scale=0.32]{images/CSR-LIL-tree.pdf}\>%
\label{CSR-tree}}
\subfloat[DCSR]{\>\includegraphics[scale=0.32]{images/DCSR-tree.pdf}%
\label{DCSR-tree}}
\subfloat[DIA-variant]{\>\includegraphics[scale=0.32]{images/DIA-variant-tree.pdf}\>
\label{DIA-variant-tree}}
\hfil
\subfloat[DIA]{\>\includegraphics[scale=0.32]{images/DIA-tree.pdf}\>
\label{DIA-tree}}
\subfloat[BCSR]{\>\includegraphics[scale=0.32]{images/BCSR-tree.pdf}\>
\label{BCSR-tree}}
\hfil
\subfloat[CSB]{\>\includegraphics[scale=0.32]{images/CSB-tree.pdf}%
\label{CSB-tree}}
\subfloat[ELLPACK]{\>\includegraphics[scale=0.32]{images/ELL-tree.pdf}%
\label{ELL-tree}}
\subfloat[C\textsuperscript{2}SR]{\>\includegraphics[scale=0.32]{images/C2SR-CPSR-tree.pdf}%
\label{C2SR-CPSR-tree}}
\hfil
\subfloat[CISR]{\>\includegraphics[scale=0.32]{images/CISR-tree.pdf}%
\label{CISR-tree}}
\subfloat[Hybrid BDIA/CSR]{\>\includegraphics[scale=0.32]{images/BDIA-CSR-tree.pdf}%
\label{BDIA-CSR-tree}}
\subfloat[Hybrid BELL/COO]{\>\includegraphics[scale=0.32]{images/BELL-COO-tree.pdf}%
\label{BELL-COO-tree}}
\hfil
% \vspace{-2pt}
\caption{The {\Tree}s of the matrix $A$ in Figure \ref{matrix} --- Yellow-shaded blocks refer to the data structure of the same tensor element. The root of a \Tree is the symbol of the tensor. $A_0$ and $A_1$ are sub-matrices of the matrix $A$. The circular nodes are metadata nodes that contain indices, and the arrows represent pointers from a higher major dimension to a lower one. Index expressions are on the left of each coordinate level. Nodes with dashed lines are elements padded for memory alignment.}
% % \zz{Section}}
\label{fig-index-tree}
\vspace{-10pt}
\end{figure*}

==> figs-tabs/fig-spgemm-csr-csr-csr.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{images/spgemm_csr-csr-csr.pdf}
    \caption{Normalized run time comparison of SpGEMM kernel across \IRName, MLIR SparseTensor Dialect, TACO, and Intel MKL using CSR format for all input and output sparse matrices. \lstinline{GM} is short for Geomean.}
    \label{fig:spgemm}
\end{figure}

==> figs-tabs/fig-storage-short.tex <==
\begin{figure*}[ht]
    \centering
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[scale=0.35]{images/matrix.pdf}
        \caption{A 5x4 matrix $A$}
        \label{matrix}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[scale=0.35]{images/COO-storage.pdf}
        \caption{COO}
        \label{COO}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[scale=0.35]{images/CSR-storage.pdf}
        \caption{CSR}
        \label{CSR}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[scale=0.35]{images/DCSR-storage.pdf}
        \caption{DCSR}
        \label{DCSR}
    \end{subfigure}
    \begin{subfigure}{0.26\textwidth}
        \centering
        \includegraphics[scale=0.35]{images/LIL-storage.pdf}
        \caption{LIL}
        \label{LIL}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[scale=0.35]{images/DOK-storage.pdf}
        \caption{DOK}
        \label{DOK}
    \end{subfigure}
    \begin{subfigure}{0.22\textwidth}
        \centering
        \includegraphics[scale=0.35]{images/DIA-storage.pdf}
        \caption{DIA}
        \label{DIA}
    \end{subfigure}
    \begin{subfigure}{0.22\textwidth}
        \centering
        \includegraphics[scale=0.35]{images/DIA-variant-storage.pdf}
        \caption{DIA-variant}
        \label{DIA-variant}
    \end{subfigure}
    \begin{subfigure}{0.2\textwidth}
        \centering
        \includegraphics[scale=0.35]{images/BCSR-storage.pdf}
        \caption{BCSR}
        \label{BCSR}
    \end{subfigure}
    \begin{subfigure}{0.28\textwidth}
        \centering
        \includegraphics[scale=0.35]{images/CSB-storage.pdf}
        \caption{CSB}
        \label{CSB}
    \end{subfigure}
    \begin{subfigure}{0.23\textwidth}
        \centering
        \includegraphics[scale=0.35]{images/ELL-indirect-storage.pdf}
        \caption{ELL}
        \label{ELL}
    \end{subfigure}
    \begin{subfigure}{0.26\textwidth}
        \centering
        \includegraphics[scale=0.35]{images/C2SR-storage.pdf}
        \caption{C\textsuperscript{2}SR (2 banks)}
        \label{C2SR}
    \end{subfigure}
    \begin{subfigure}{0.28\textwidth}
        \centering
        \includegraphics[scale=0.35]{images/CISR-indirect-storage.pdf}
        \caption{CISR (2 banks)}
        \label{CISR}
    \end{subfigure}
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[scale=0.35]{images/BDIA-CSR-storage.pdf}
        \caption{Hybrid BDIA/CSR}
        \label{BDIA-CSR}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[scale=0.35]{images/BELL-COO-indirect-storage.pdf}
        \caption{Hybrid BELL/COO}
        \label{BELL-COO}
    \end{subfigure}
    \vspace{-8pt}
    \caption{Different formats of a sparse matrix ($A$) --- Yellow-shaded blocks refer to the data structure of the same tensor element. The \textit{size}, \textit{ptr}, \textit{idx}, and \textit{val} labels on the left indicate the size of a dimension, a pointer array, an index array, or a value array. The index expressions on the right denote the \Map at each level. Horizontal dotted lines separate different tensor dimensions, while vertical dotted lines divide the matrix $A$ into sub-matrices. 
    % \rh{Figure 1e and 1f: why coloring value 3? }
    }
    % Connected elements are stored contiguously in memory. 
    \label{fig:format-storage}
    \vspace{-8pt}
\end{figure*}
% \Arrays labeled with \textit{indirect} map functions are blurred and not explicitly stored in memory. 

==> figs-tabs/tab-BDIA-breakdown.tex <==
\begin{table}[ht]%[tb!]
\centering
% \vspace{-5pt}
\caption{The breakdown execution time (in seconds) of operators when converting from COO to BDIA.}
% \vspace{-5pt}
\footnotesize
\setlength\tabcolsep{5pt} % Reduce the white space margins in each cell
\lstset{%
tabsize=2,
columns=fullflexible,
basicstyle=\ttfamily\scriptsize,
breaklines=true,
breakatwhitespace,
escapeinside={(*}{*)},
alsoletter={\., \_},
morekeywords={tile\_division, tile\_union, enumerate, reorder, schedule, move\_lv, trim, fill, merge, split, vectorize, devectorize, pad, pack, partition}
}
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{c|cccccccccc}
\toprule
 & Total & swap & sub & tile\_split & move & move & fuse & fuse & grow & vectorize \\\hline
 ge & 1 (8.923) & 0.00\% & 0.62\% & 10.17\% & 16.94\% & 57.54\% & 4.52\% & 5.84\% & 0.00\% & 4.36\% \\
 ss & 1 (0.967) & 0.00\% & 0.95\% & 18.27\% & 25.90\% & 34.71\% & 7.09\% & 8.20\% & 0.01\% & 4.86\% \\
 ra & 1 (2.094) & 0.00\% & 1.05\% & 16.72\% & 26.70\% & 34.26\% & 7.78\% & 7.58\% & 0.01\% & 5.88\% \\
 mc & 1 (1.524) & 0.00\% & 1.16\% & 17.18\% & 28.51\% & 32.29\% & 8.30\% & 8.55\% & 0.02\% & 0.10\% \\
 vs & 1 (0.616) & 0.00\% & 1.00\% & 17.74\% & 26.62\% & 34.36\% & 7.05\% & 8.26\% & 0.01\% & 4.95\% \\
 lp & 1 (1.405) & 0.00\% & 0.67\% & 11.12\% & 18.24\% & 56.00\% & 4.80\% & 5.73\% & 0.00\% & 3.44\% \\
 tp & 1 (0.272) & 0.00\% & 0.99\% & 16.10\% & 37.11\% & 37.15\% & 7.10\% & 8.31\% & 0.01\% & 3.22\% \\
 ts & 1 (0.559) & 0.00\% & 0.67\% & 11.16\% & 18.16\% & 56.25\% & 4.79\% & 5.69\% & 0.00\% & 3.28\% \\\midrule
 GM & 1         & 0.00\% & 0.90\% & 14.98\% & 23.86\% & 39.79\% & 6.51\% & 7.40\% & 0.01\% & 2.54\% \\
\bottomrule
\end{tabular}
}
\label{tab:bdia-breakdown}
\vspace{-10pt}
\end{table}

==> figs-tabs/tab-codegen-stdv.tex <==
\begin{table}[ht]%[tb!]
\centering
% \vspace{-5pt}
\caption{
Comparison of normalized execution times for compute kernels generated by \IRName, \newrev{the MLIR SparseTensor dialect under the LLVM 15.0.0 release}, and \newrev{the main branch of TACO~\cite{github_taco}}, relative to the performance achieved by \IRName. The actual execution times (in \textit{seconds}) for compute kernels generated by \IRName are shown in parentheses. \newrev{The numbers for each execution time $\pm$ standard deviation are computed based on 20 independent runs.}}
\footnotesize
\setlength\tabcolsep{5pt} % Reduce the white space margins in each cell
\lstset{%
tabsize=2,
columns=fullflexible,
basicstyle=\ttfamily\scriptsize,
breaklines=true,
breakatwhitespace,
escapeinside={(*}{*)},
alsoletter={\., \_},
morekeywords={tile\_division, tile\_union, enumerate, reorder, schedule, move\_lv, trim, fill, merge, split, vectorize, devectorize, pad, pack, partition}
}
\resizebox{0.95\textwidth}{!}{\newtablerev
\begin{tabular}{c|ccc|ccc|c|c}
\toprule
\multirow{2}{*}{\makecell{\thead{\textbf{Data}}}} & \multicolumn{3}{c|}{\thead{\textbf{CSR SpMM}}} & \multicolumn{3}{c|}{\thead{\textbf{DCSC SpMM}}}  & \multirow{2}{*}{\makecell{\thead{\textbf{Data}}}} & \multicolumn{1}{c}{\thead{\textbf{DIA-variant}\\\textbf{SpMM}}} \\
\cmidrule{2-7} \cmidrule{9-9}
    & \IRName & \makecell{SparseTensor} & TACO & \IRName & \makecell{SparseTensor} & TACO &  & \IRName  \\\midrule
   m2    & 1 (1.847 $\pm$ 0.038) & 1.049 $\pm$ 0.167 & 5.243 $\pm$ 0.059 & 1 (1.857 $\pm$ 0.018) & 1.017 $\pm$ 0.046 & 5.173 $\pm$ 0.032 & bw &  (0.078 $\pm$ 0.001)  \\
   sc    & 1 (0.734 $\pm$ 0.042) & 0.991 $\pm$ 0.006 & 5.917 $\pm$ 0.063 & 1 (0.730 $\pm$ 0.007) & 1.013 $\pm$ 0.047 & 6.044 $\pm$ 0.431 & af &  (8.136 $\pm$ 0.135)  \\
   pg    & 1 (0.153 $\pm$ 0.006) & 1.007 $\pm$ 0.013 & 5.744 $\pm$ 0.062 & 1 (0.150 $\pm$ 0.002) & 1.009 $\pm$ 0.038 & 5.851 $\pm$ 0.074 & cg &  (0.528 $\pm$ 0.012)  \\
   ca    & 1 (1.498 $\pm$ 0.030) & 1.024 $\pm$ 0.013 & 5.449 $\pm$ 0.330 & 1 (1.528 $\pm$ 0.027) & 1.026 $\pm$ 0.041 & 5.224 $\pm$ 0.053 & ex & (22.642 $\pm$ 0.323)  \\
   f3    & 1 (1.702 $\pm$ 0.059) & 1.028 $\pm$ 0.082 & 6.066 $\pm$ 0.080 & 1 (1.729 $\pm$ 0.038) & 1.021 $\pm$ 0.032 & 5.297 $\pm$ 0.046 & cm &  (2.026 $\pm$ 0.027) \\
   cc    & 1 (0.187 $\pm$ 0.009) & 0.990 $\pm$ 0.021 & 4.370 $\pm$ 0.059 & 1 (0.187 $\pm$ 0.003) & 1.009 $\pm$ 0.030 & 4.360 $\pm$ 0.041 & ct & (32.896 $\pm$ 0.460)  \\
   p3    & 1 (0.302 $\pm$ 0.021) & 0.990 $\pm$ 0.023 & 4.524 $\pm$ 0.067 & 1 (0.302 $\pm$ 0.006) & 1.000 $\pm$ 0.020 & 4.472 $\pm$ 0.045 & nm &  (7.841 $\pm$ 0.133)  \\
   ee    & 1 (0.014 $\pm$ 0.001) & 1.013 $\pm$ 0.087 & 7.139 $\pm$ 0.151 & 1 (0.014 $\pm$ 0.001) & 1.037 $\pm$ 0.092 & 7.247 $\pm$ 0.141 & ee &  (3.806 $\pm$ 0.044)  \\
   ch    & 1 (0.136 $\pm$ 0.009) & 0.977 $\pm$ 0.052 & 6.774 $\pm$ 0.049 & 1 (0.135 $\pm$ 0.008) & 1.008 $\pm$ 0.061 & 6.809 $\pm$ 0.055 & ch &  (2.179 $\pm$ 0.084) \\
   sh    & 1 (0.223 $\pm$ 0.016) & 0.998 $\pm$ 0.066 & 6.989 $\pm$ 0.037 & 1 (0.222 $\pm$ 0.002) & 1.034 $\pm$ 0.069 & 7.039 $\pm$ 0.056 & sh &  (5.821 $\pm$ 0.202)  \\
   mj    & 1 (1.133 $\pm$ 0.124) & 1.028 $\pm$ 0.173 & 6.177 $\pm$ 0.043 & 1 (1.125 $\pm$ 0.024) & 0.979 $\pm$ 0.023 & 6.216 $\pm$ 0.046 & mj & (30.623 $\pm$ 0.472)  \\
   bm    & 1 (0.542 $\pm$ 0.049) & 0.983 $\pm$ 0.058 & 6.024 $\pm$ 0.020 & 1 (0.529 $\pm$ 0.005) & 1.032 $\pm$ 0.080 & 6.191 $\pm$ 0.046 & bm & ( 8.672 $\pm$ 0.235) \\\midrule
 Geomean & 1                     & 1.006             & 5.805             & 1                     & 1.015             & 5.809   &    &   \\
\bottomrule
\end{tabular}
}
\begin{adjustwidth}{0.33cm}{}
% \begin{adjustbox}{width=.67\textwidth,left}
\resizebox{0.67\textwidth}{!}{\newtablerev
\begin{tabular}{c|ccc|cc}
\toprule
\multirow{2}{*}{\makecell{\thead{\textbf{Data}}}} & \multicolumn{3}{c|}{\thead{\textbf{CSR}{$\times$}\textbf{CSR}$\rightarrow$\textbf{CSR}\\\textbf{SpGEMM}}} & \multicolumn{2}{c}{\thead{\textbf{CSC}{$\times$}\textbf{CSC}$\rightarrow$\textbf{CSC}\\\textbf{SpGEMM}}} \\
\cmidrule{2-6}
    & \IRName  & \makecell{SparseTensor} & TACO & \IRName & \makecell{SparseTensor} \\\midrule
   m2    & 1 (0.305 $\pm$ 0.006) & 1.278 $\pm$ 0.014 & 2.001 $\pm$ 0.034 & 1 (0.309 $\pm$ 0.006) & 1.254 $\pm$ 0.015 \\
   sc    & 1 (0.242 $\pm$ 0.003) & 1.013 $\pm$ 0.009 & 1.791 $\pm$ 0.012 & 1 (0.244 $\pm$ 0.008) & 1.002 $\pm$ 0.012 \\
   pg    & 1 (0.028 $\pm$ 0.001) & 1.148 $\pm$ 0.038 & 1.817 $\pm$ 0.064 & 1 (0.025 $\pm$ 0.001) & 1.200 $\pm$ 0.025 \\
   ca    & 1 (0.657 $\pm$ 0.014) & 1.104 $\pm$ 0.011 & 2.108 $\pm$ 0.015 & 1 (0.654 $\pm$ 0.006) & 1.101 $\pm$ 0.018 \\
   f3    & 1 (1.058 $\pm$ 0.008) & 1.113 $\pm$ 0.016 & 1.929 $\pm$ 0.016 & 1 (1.062 $\pm$ 0.008) & 1.098 $\pm$ 0.010 \\
   cc    & 1 (0.137 $\pm$ 0.001) & 1.064 $\pm$ 0.013 & 1.953 $\pm$ 0.031 & 1 (0.137 $\pm$ 0.002) & 1.048 $\pm$ 0.013 \\
   p3    & 1 (0.179 $\pm$ 0.003) & 1.070 $\pm$ 0.015 & 2.157 $\pm$ 0.027 & 1 (0.178 $\pm$ 0.002) & 1.062 $\pm$ 0.013 \\
   ee    & 1 (0.020 $\pm$ 0.001) & 1.077 $\pm$ 0.081 & 2.800 $\pm$ 0.257 & 1 (0.019 $\pm$ 0.001) & 1.058 $\pm$ 0.049 \\
   ch    & 1 (0.012 $\pm$ 0.001) & 0.991 $\pm$ 0.070 & 2.843 $\pm$ 0.123 & 1 (0.013 $\pm$ 0.000) & 0.903 $\pm$ 0.011 \\
   sh    & 1 (0.020 $\pm$ 0.001) & 1.037 $\pm$ 0.123 & 2.385 $\pm$ 0.073 & 1 (0.021 $\pm$ 0.004) & 0.914 $\pm$ 0.017 \\
   mj    & 1 (0.219 $\pm$ 0.015) & 1.146 $\pm$ 0.101 & 2.297 $\pm$ 0.028 & 1 (0.217 $\pm$ 0.001) & 1.118 $\pm$ 0.059 \\
   bm    & 1 (0.079 $\pm$ 0.007) & 1.011 $\pm$ 0.078 & 1.966 $\pm$ 0.018 & 1 (0.077 $\pm$ 0.005) & 1.001 $\pm$ 0.050 \\\midrule
Geomean  & 1                     & 1.085             & 2.146             & 1                     & 1.059             \\
\bottomrule
\end{tabular}
}
% \end{adjustbox}
\end{adjustwidth}
\label{tab:codegen}
\end{table}
 

==> figs-tabs/tab-codegen.tex <==
\begin{table}[ht]%[tb!]
\centering
% \vspace{-5pt}
\caption{
\rev{Comparison of normalized execution times for compute kernels generated by \IRName, MLIR SparseTensor dialect, and \newrev{the main branch of TACO~\cite{github_taco}}, relative to the performance achieved by \IRName. The actual execution times (in \textit{seconds}) for compute kernels generated by \IRName are shown in parentheses. }}
\footnotesize
\setlength\tabcolsep{5pt} % Reduce the white space margins in each cell
\lstset{%
tabsize=2,
columns=fullflexible,
basicstyle=\ttfamily\scriptsize,
breaklines=true,
breakatwhitespace,
escapeinside={(*}{*)},
alsoletter={\., \_},
morekeywords={tile\_division, tile\_union, enumerate, reorder, schedule, move\_lv, trim, fill, merge, split, vectorize, devectorize, pad, pack, partition}
}
\resizebox{\textwidth}{!}{\tablerev
\begin{tabular}{c|ccc|ccc|ccc|cc}
\toprule
\multirow{2}{*}{\makecell{\thead{\textbf{Data}}}} & \multicolumn{3}{c|}{\thead{\textbf{CSR SpMM}}} & \multicolumn{3}{c|}{\thead{\textbf{DCSC SpMM}}} & \multicolumn{3}{c|}{\thead{\textbf{CSR}{$\times$}\textbf{CSR}$\rightarrow$\textbf{CSR}\\\textbf{SpGEMM}}} & \multicolumn{2}{c}{\thead{\textbf{CSC}{$\times$}\textbf{CSC}$\rightarrow$\textbf{CSC}\\\textbf{SpGEMM}}} \\
\cmidrule{2-12} 
    & \IRName & \makecell{SparseTensor} & TACO & \IRName & \makecell{SparseTensor} & TACO & \IRName & \makecell{SparseTensor} & TACO & \IRName & \makecell{SparseTensor} \\\midrule
wg & 1 (5.321) & 1.06 & 1.37 & 1 (5.638) & 1.05 & 1.38 & 1 (2.300) & 1.15 & 1.77 & 1 (2.176) & 1.18 \\
m2 & 1 (1.765) & 1.04 & 1.52 & 1 (1.719) & 1.07 & 1.62 & 1 (0.260) & 1.37 & 2.09 & 1 (0.271) & 1.21 \\
az & 1 (2.711) & 1.05 & 1.27 & 1 (2.741) & 1.05 & 1.39 & 1 (0.760) & 1.28 & 2.06 & 1 (0.888) & 1.08 \\
sc & 1 (0.697) & 1.01 & 2.49 & 1 (0.665) & 1.06 & 1.73 & 1 (0.223) & 1.06 & 1.85 & 1 (0.232) & 0.96 \\
pg & 1 (0.133) & 1.08 & 2.46 & 1 (0.132) & 1.06 & 2.47 & 1 (0.025) & 1.35 & 1.82 & 1 (0.023) & 1.13 \\
ca & 1 (1.452) & 0.99 & 1.07 & 1 (1.393) & 1.03 & 1.18 & 1 (0.612) & 1.14 & 2.18 & 1 (0.602) & 1.10 \\
cs & 1 (1.042) & 0.93 & 1.01 & 1 (0.952) & 1.03 & 1.24 & 1 (0.500) & 1.09 & 2.18 & 1 (0.517) & 0.99 \\
f3 & 1 (1.691) & 0.91 & 0.91 & 1 (1.538) & 1.01 & 1.11 & 1 (1.008) & 1.15 & 1.97 & 1 (1.007) & 1.09 \\
cc & 1 (0.165) & 1.00 & 1.40 & 1 (0.165) & 1.04 & 1.37 & 1 (0.128) & 1.15 & 2.01 & 1 (0.142) & 0.93 \\
wv & 1 (0.060) & 0.91 & 1.27 & 1 (0.054) & 1.00 & 1.62 & 1 (0.088) & 1.12 & 2.27 & 1 (0.096) & 1.02 \\
p3 & 1 (0.268) & 1.01 & 1.04 & 1 (0.268) & 1.04 & 1.06 & 1 (0.164) & 1.11 & 2.27 & 1 (0.163) & 1.02 \\
ee & 1 (0.014) & 0.88 & 1.27 & 1 (0.012) & 1.24 & 1.55 & 1 (0.018) & 1.10 & 2.82 & 1 (0.018) & 1.03 \\\midrule
 Geomean & 1  & 0.99 & 1.35 & 1        & 1.06 & 1.44   & 1         & 1.17 & 2.09 & 1         & 1.06 \\
 % Geomean & 1  & 1.02  & 1.34  & 1   & 0.86 & 1.39 & 1 & 1.01 &  1.50  & 1  & 1.01  & 1.46  & 1  & 1.02  & 1.34  & 1   & 0.86 & 1.39 & 1 & 1.01 &  1.50  & 1  & 1.01  & 1.46  \\
\bottomrule
\end{tabular}
}
\label{tab:codegen}
\end{table}
 % wv & 1 (0.001) & 2.98   & 1.50  & 1 (0.080) & 1.11 & 1 (0.016) & 1.19 & (0.019) & (0.065) & (0.004) & (0.004) \\
 % ee & 1 (0.000) & 11.18  & 3.00  & 1 (0.004) & 1.10 & 1 (0.001) & 1.23 & (0.003) & (0.004) & (0.001) & (0.001) \\
 % nm & 1 (0.002) & 14.43  & 2.63  & 1 (0.004) & 2.16 & 1 (0.005) & 1.70 & (0.038) & (0.030) & (0.019) & (0.018) \\
 % cm & 1 (0.001) & 8.16   & 1.71  & 1 (0.001) & 1.33 & 1 (0.002) & 1.44 & (0.014) & (0.009) & (0.006) & (0.007) \\
 % ct & 1 (0.010) & 8.17   & 1.79  & 1 (0.014) & 2.40 & 1 (0.022) & 1.97 & (0.151) & (0.169) & (0.070) & (0.074) \\
 % lp & 1 (0.185) & 3.56   & 0.92  & 1 (0.377) & 1.09 & 1 (0.270) & 1.22 & (2.634) & (4.352) & (1.106) & (1.114) \\
 % tp & 1 (0.131) & 4.25   & 1.11  & 1 (0.139) & 0.99 & 1 (0.216) & 0.91 & (2.335) & (5.584) & (0.943) & (1.303) \\
 % ts & 1 (0.152) & 3.00   & 0.97  & 1 (0.168) & 1.11 & 1 (0.230) & 1.10 & (1.651) & (2.319) & (0.558) & (0.523) \\
 % ch & 1 (0.001) & 4.65   & 0.60  & 1 (0.001) & 0.89 & 1 (0.002) & 0.53 & (0.017) & (0.012) & (0.008) & (0.010) \\
 % mj & 1 (0.008) & 5.47   & 0.76  & 1 (0.009) & 1.11 & 1 (0.016) & 0.58 & (0.130) & (0.153) & (0.057) & (0.068) \\
 % sh & 1 (0.002) & 5.36   & 0.63  & 1 (0.002) & 1.19 & 1 (0.003) & 0.72 & (0.023) & (0.017) & (0.013) & (0.014) \\
 % bm & 1 (0.003) & 7.10   & 0.92  & 1 (0.004) & 0.78 & 1 (0.003) & 1.28 & (0.054) & (0.060) & (0.025) & (0.031) \\\midrule

==> figs-tabs/tab-conversion-stdv-opt-v2.tex <==
\begin{table}[ht]%[tb!]
\centering
% \vspace{-5pt}
\caption{
Comparison of normalized execution times for format conversion programs generated by \IRName, \newrev{the MLIR SparseTensor dialect under the LLVM 15.0.0 release}, and \rev{the format conversion artifact of} TACO~\cite{github_chou2020automatic}, relative to the performance achieved by \IRName. The actual execution times (in \textit{seconds}) for format conversion programs generated by \IRName are shown in parentheses. \newrev{The numbers for each execution time $\pm$ standard deviation are computed based on 20 independent runs.}
}
% \vspace{-5pt}
\footnotesize
\setlength\tabcolsep{5pt} % Reduce the white space margins in each cell
\lstset{%
tabsize=2,
columns=fullflexible,
basicstyle=\ttfamily\scriptsize,
breaklines=true,
breakatwhitespace,
escapeinside={(*}{*)},
alsoletter={\., \_},
morekeywords={tile\_division, tile\_union, enumerate, reorder, schedule, move\_lv, trim, fill, merge, split, vectorize, devectorize, pad, pack, partition}
}
\resizebox{0.8\textwidth}{!}{\newtablerev
\begin{tabular}{c|ccc|c|c}
\toprule
\multirow{2}{*}{\makecell{\textbf{Data}}} & \multicolumn{3}{c|}{\textbf{CSR} $\rightarrow$ \textbf{CSC}} & \textbf{DCSC} $\rightarrow$ \textbf{BCSR} & \textbf{CSB} $\rightarrow$ \textbf{DIA-variant}  \\
\cmidrule{2-6} 
    & \IRName & \makecell{SparseTensor} & TACO & \IRName & \IRName  \\\midrule
 wv & 1 (0.001 $\pm$ 0.000) &  3.962 $\pm$ 0.391 & 1.448 $\pm$ 0.055 & 0.012 $\pm$ 0.001 & (0.067 $\pm$ 0.001)  \\
 ee & 1 (0.000 $\pm$ 0.000) &  5.075 $\pm$ 0.660 & 1.259 $\pm$ 0.065 & 0.003 $\pm$ 0.000 & (0.004 $\pm$ 0.000)  \\
 nm & 1 (0.002 $\pm$ 0.000) & 14.594 $\pm$ 0.366 & 2.474 $\pm$ 0.030 & 0.039 $\pm$ 0.000 & (0.032 $\pm$ 0.001)  \\
 cm & 1 (0.001 $\pm$ 0.000) & 10.042 $\pm$ 0.559 & 1.828 $\pm$ 0.021 & 0.012 $\pm$ 0.001 & (0.007 $\pm$ 0.000)  \\
 ct & 1 (0.009 $\pm$ 0.000) &  8.955 $\pm$ 0.449 & 2.012 $\pm$ 0.014 & 0.148 $\pm$ 0.001 & (0.184 $\pm$ 0.002)  \\
 lp & 1 (0.193 $\pm$ 0.003) &  3.416 $\pm$ 0.025 & 0.991 $\pm$ 0.021 & 2.554 $\pm$ 0.015 & (4.509 $\pm$ 0.031)  \\
 tp & 1 (0.139 $\pm$ 0.002) &  4.039 $\pm$ 0.032 & 1.205 $\pm$ 0.025 & 2.249 $\pm$ 0.010 & (6.157 $\pm$ 0.038)  \\
 ts & 1 (0.168 $\pm$ 0.001) &  2.747 $\pm$ 0.034 & 0.966 $\pm$ 0.013 & 1.733 $\pm$ 0.009 & (2.509 $\pm$ 0.017)  \\
 ch & 1 (0.001 $\pm$ 0.000) &  6.253 $\pm$ 0.067 & 0.637 $\pm$ 0.017 & 0.015 $\pm$ 0.001 & (0.009 $\pm$ 0.000)  \\
 mj & 1 (0.008 $\pm$ 0.000) &  5.148 $\pm$ 0.072 & 0.748 $\pm$ 0.006 & 0.134 $\pm$ 0.001 & (0.178 $\pm$ 0.002)  \\
 sh & 1 (0.001 $\pm$ 0.000) &  5.871 $\pm$ 0.667 & 0.637 $\pm$ 0.009 & 0.023 $\pm$ 0.000 & (0.018 $\pm$ 0.000)  \\
 bm & 1 (0.003 $\pm$ 0.000) &  6.025 $\pm$ 0.110 & 0.753 $\pm$ 0.006 & 0.058 $\pm$ 0.001 & (0.063 $\pm$ 0.001)  \\\midrule
 Geomean & 1                &  5.685             & 1.131              &                                 &      \\
\bottomrule
\end{tabular}
}
\begin{adjustwidth}{0.828cm}{}
\resizebox{0.8\textwidth}{!}{\newtablerev
% \relscale{0.5}
% \fontsize{3pt}{1pt}\selectfont
% \setlength\tabcolsep{3pt} % Reduce the white space margins in each cell
\begin{tabular}{c|cc|cc|c|c}
\toprule
\multirow{2}{*}{\makecell{\textbf{Data}}} & \multicolumn{2}{c|}{\textbf{COO} $\rightarrow$ \textbf{ELL}} & \multicolumn{2}{c|}{\textbf{COO} $\rightarrow$ \textbf{DIA}} & \textbf{COO} $\rightarrow$ \textbf{C\textsuperscript{2}SR} & \textbf{COO} $\rightarrow$ \textbf{CISR}\\
\cmidrule{2-7} 
    & \IRName & TACO & \IRName & TACO & \IRName & \IRName \\\midrule
 wv & 1 (0.014 $\pm$ 0.001) & 1.285 $\pm$ 0.024 & 1 (0.065 $\pm$ 0.004) & 1.404 $\pm$ 0.013 & 0.003 $\pm$ 0.000 & 0.003 $\pm$ 0.000 \\
 ee & 1 (0.001 $\pm$ 0.000) & 1.185 $\pm$ 0.046 & 1 (0.003 $\pm$ 0.000) & 1.609 $\pm$ 0.066 & 0.001 $\pm$ 0.000 & 0.001 $\pm$ 0.000 \\
 nm & 1 (0.006 $\pm$ 0.000) & 1.842 $\pm$ 0.045 & 1 (0.003 $\pm$ 0.000) & 2.394 $\pm$ 0.025 & 0.017 $\pm$ 0.000 & 0.017 $\pm$ 0.000 \\
 cm & 1 (0.002 $\pm$ 0.000) & 1.357 $\pm$ 0.026 & 1 (0.001 $\pm$ 0.000) & 1.631 $\pm$ 0.020 & 0.005 $\pm$ 0.000 & 0.005 $\pm$ 0.000 \\
 ct & 1 (0.023 $\pm$ 0.000) & 2.107 $\pm$ 0.015 & 1 (0.013 $\pm$ 0.000) & 2.356 $\pm$ 0.032 & 0.071 $\pm$ 0.001 & 0.077 $\pm$ 0.001 \\
 lp & 1 (0.298 $\pm$ 0.005) & 0.970 $\pm$ 0.020 & 1 (0.352 $\pm$ 0.008) & 1.231 $\pm$ 0.012 & 1.069 $\pm$ 0.004 & 1.080 $\pm$ 0.021 \\
 tp & 1 (0.220 $\pm$ 0.002) & 0.945 $\pm$ 0.024 & 1 (0.127 $\pm$ 0.002) & 1.043 $\pm$ 0.025 & 0.929 $\pm$ 0.009 & 1.303 $\pm$ 0.062 \\
 ts & 1 (0.249 $\pm$ 0.004) & 1.098 $\pm$ 0.013 & 1 (0.163 $\pm$ 0.002) & 1.176 $\pm$ 0.011 & 0.541 $\pm$ 0.005 & 0.508 $\pm$ 0.045 \\
 ch & 1 (0.002 $\pm$ 0.000) & 0.551 $\pm$ 0.009 & 1 (0.001 $\pm$ 0.000) & 0.974 $\pm$ 0.019 & 0.006 $\pm$ 0.001 & 0.007 $\pm$ 0.001 \\
 mj & 1 (0.017 $\pm$ 0.000) & 0.570 $\pm$ 0.005 & 1 (0.008 $\pm$ 0.000) & 1.221 $\pm$ 0.015 & 0.060 $\pm$ 0.001 & 0.072 $\pm$ 0.001 \\
 sh & 1 (0.003 $\pm$ 0.000) & 0.845 $\pm$ 0.006 & 1 (0.001 $\pm$ 0.000) & 1.434 $\pm$ 0.019 & 0.011 $\pm$ 0.000 & 0.013 $\pm$ 0.000 \\
 bm & 1 (0.007 $\pm$ 0.000) & 0.549 $\pm$ 0.005 & 1 (0.004 $\pm$ 0.000) & 0.813 $\pm$ 0.007 & 0.026 $\pm$ 0.000 & 0.031 $\pm$ 0.000 \\\midrule
 Geomean & 1                & 1.014  & 1                     & 1.369             &                     &                     \\
\bottomrule
\end{tabular}
}
\end{adjustwidth}
\label{tab:conversion}
% \vspace{-5pt}
\end{table}



==> figs-tabs/tab-conversion-stdv-opt.tex <==
\begin{table}[ht]%[tb!]
\centering
% \vspace{-5pt}
\caption{
Comparison of normalized execution times for format conversion programs generated by \IRName, \newrev{the MLIR SparseTensor dialect under the LLVM 15.0.0 release}, and \rev{the format conversion artifact of} TACO~\cite{github_chou2020automatic}, relative to the performance achieved by \IRName. The actual execution times (in \textit{seconds}) for format conversion programs generated by \IRName are shown in parentheses. \newrev{The numbers for each execution time $\pm$ standard deviation are computed based on 20 independent runs.}
}
% \vspace{-5pt}
\footnotesize
\setlength\tabcolsep{5pt} % Reduce the white space margins in each cell
\lstset{%
tabsize=2,
columns=fullflexible,
basicstyle=\ttfamily\scriptsize,
breaklines=true,
breakatwhitespace,
escapeinside={(*}{*)},
alsoletter={\., \_},
morekeywords={tile\_division, tile\_union, enumerate, reorder, schedule, move\_lv, trim, fill, merge, split, vectorize, devectorize, pad, pack, partition}
}
\resizebox{0.88\textwidth}{!}{\newtablerev
\begin{tabular}{c|ccc|cc|c}
\toprule
\multirow{2}{*}{\makecell{\textbf{Data}}} & \multicolumn{3}{c|}{\textbf{CSR} $\rightarrow$ \textbf{CSC}} & \multicolumn{2}{c|}{\textbf{COO} $\rightarrow$ \textbf{DIA}} & \textbf{CSB} $\rightarrow$ \textbf{DIA-variant}  \\
\cmidrule{2-7} 
    & \IRName & \makecell{SparseTensor} & TACO & \IRName & TACO & \IRName  \\\midrule
 wv & 1 (0.001 $\pm$ 0.000) &  3.962 $\pm$ 0.391 & 1.448 $\pm$ 0.055 & 1 (0.065 $\pm$ 0.004) & 1.404 $\pm$ 0.013 & (0.067 $\pm$ 0.001)  \\
 ee & 1 (0.000 $\pm$ 0.000) &  5.075 $\pm$ 0.660 & 1.259 $\pm$ 0.065 & 1 (0.003 $\pm$ 0.000) & 1.609 $\pm$ 0.066 & (0.004 $\pm$ 0.000)  \\
 nm & 1 (0.002 $\pm$ 0.000) & 14.594 $\pm$ 0.366 & 2.474 $\pm$ 0.030 & 1 (0.003 $\pm$ 0.000) & 2.394 $\pm$ 0.025 & (0.032 $\pm$ 0.001)  \\
 cm & 1 (0.001 $\pm$ 0.000) & 10.042 $\pm$ 0.559 & 1.828 $\pm$ 0.021 & 1 (0.001 $\pm$ 0.000) & 1.631 $\pm$ 0.020 & (0.007 $\pm$ 0.000)  \\
 ct & 1 (0.009 $\pm$ 0.000) &  8.955 $\pm$ 0.449 & 2.012 $\pm$ 0.014 & 1 (0.013 $\pm$ 0.000) & 2.356 $\pm$ 0.032 & (0.184 $\pm$ 0.002)  \\
 lp & 1 (0.193 $\pm$ 0.003) &  3.416 $\pm$ 0.025 & 0.991 $\pm$ 0.021 & 1 (0.352 $\pm$ 0.008) & 1.231 $\pm$ 0.012 & (4.509 $\pm$ 0.031)  \\
 tp & 1 (0.139 $\pm$ 0.002) &  4.039 $\pm$ 0.032 & 1.205 $\pm$ 0.025 & 1 (0.127 $\pm$ 0.002) & 1.043 $\pm$ 0.025 & (6.157 $\pm$ 0.038)  \\
 ts & 1 (0.168 $\pm$ 0.001) &  2.747 $\pm$ 0.034 & 0.966 $\pm$ 0.013 & 1 (0.163 $\pm$ 0.002) & 1.176 $\pm$ 0.011 & (2.509 $\pm$ 0.017)  \\
 ch & 1 (0.001 $\pm$ 0.000) &  6.253 $\pm$ 0.067 & 0.637 $\pm$ 0.017 & 1 (0.001 $\pm$ 0.000) & 0.974 $\pm$ 0.019 & (0.009 $\pm$ 0.000)  \\
 mj & 1 (0.008 $\pm$ 0.000) &  5.148 $\pm$ 0.072 & 0.748 $\pm$ 0.006 & 1 (0.008 $\pm$ 0.000) & 1.221 $\pm$ 0.015 & (0.178 $\pm$ 0.002)  \\
 sh & 1 (0.001 $\pm$ 0.000) &  5.871 $\pm$ 0.667 & 0.637 $\pm$ 0.009 & 1 (0.001 $\pm$ 0.000) & 1.434 $\pm$ 0.019 & (0.018 $\pm$ 0.000)  \\
 bm & 1 (0.003 $\pm$ 0.000) &  6.025 $\pm$ 0.110 & 0.753 $\pm$ 0.006 & 1 (0.004 $\pm$ 0.000) & 0.813 $\pm$ 0.007 & (0.063 $\pm$ 0.001)  \\\midrule
 Geomean & 1                &  5.685             & 1.131             & 1                     & 1.369             &      \\
\bottomrule
\end{tabular}
}
\begin{adjustwidth}{0.828cm}{}
\resizebox{0.73\textwidth}{!}{\newtablerev
% \relscale{0.5}
% \fontsize{3pt}{1pt}\selectfont
% \setlength\tabcolsep{3pt} % Reduce the white space margins in each cell
\begin{tabular}{c|cc|c|c|c}
\toprule
\multirow{2}{*}{\makecell{\textbf{Data}}} & \multicolumn{2}{c|}{\textbf{COO} $\rightarrow$ \textbf{ELL}} & \textbf{DCSC} $\rightarrow$ \textbf{BCSR} & \textbf{COO} $\rightarrow$ \textbf{C\textsuperscript{2}SR} & \textbf{COO} $\rightarrow$ \textbf{CISR}\\
\cmidrule{2-6} 
    & \IRName & TACO & \IRName & \IRName & \IRName \\\midrule
 wv & 1 (0.014 $\pm$ 0.001) & 1.285 $\pm$ 0.024 & (0.012 $\pm$ 0.001) & (0.003 $\pm$ 0.000) & (0.003 $\pm$ 0.000) \\
 ee & 1 (0.001 $\pm$ 0.000) & 1.185 $\pm$ 0.046 & (0.003 $\pm$ 0.000) & (0.001 $\pm$ 0.000) & (0.001 $\pm$ 0.000) \\
 nm & 1 (0.006 $\pm$ 0.000) & 1.842 $\pm$ 0.045 & (0.039 $\pm$ 0.000) & (0.017 $\pm$ 0.000) & (0.017 $\pm$ 0.000) \\
 cm & 1 (0.002 $\pm$ 0.000) & 1.357 $\pm$ 0.026 & (0.012 $\pm$ 0.001) & (0.005 $\pm$ 0.000) & (0.005 $\pm$ 0.000) \\
 ct & 1 (0.023 $\pm$ 0.000) & 2.107 $\pm$ 0.015 & (0.148 $\pm$ 0.001) & (0.071 $\pm$ 0.001) & (0.077 $\pm$ 0.001) \\
 lp & 1 (0.298 $\pm$ 0.005) & 0.970 $\pm$ 0.020 & (2.554 $\pm$ 0.015) & (1.069 $\pm$ 0.004) & (1.080 $\pm$ 0.021) \\
 tp & 1 (0.220 $\pm$ 0.002) & 0.945 $\pm$ 0.024 & (2.249 $\pm$ 0.010) & (0.929 $\pm$ 0.009) & (1.303 $\pm$ 0.062) \\
 ts & 1 (0.249 $\pm$ 0.004) & 1.098 $\pm$ 0.013 & (1.733 $\pm$ 0.009) & (0.541 $\pm$ 0.005) & (0.508 $\pm$ 0.045) \\
 ch & 1 (0.002 $\pm$ 0.000) & 0.551 $\pm$ 0.009 & (0.015 $\pm$ 0.001) & (0.006 $\pm$ 0.001) & (0.007 $\pm$ 0.001) \\
 mj & 1 (0.017 $\pm$ 0.000) & 0.570 $\pm$ 0.005 & (0.134 $\pm$ 0.001) & (0.060 $\pm$ 0.001) & (0.072 $\pm$ 0.001) \\
 sh & 1 (0.003 $\pm$ 0.000) & 0.845 $\pm$ 0.006 & (0.023 $\pm$ 0.000) & (0.011 $\pm$ 0.000) & (0.013 $\pm$ 0.000) \\
 bm & 1 (0.007 $\pm$ 0.000) & 0.549 $\pm$ 0.005 & (0.058 $\pm$ 0.001) & (0.026 $\pm$ 0.000) & (0.031 $\pm$ 0.000) \\\midrule
 Geomean & 1                & 1.014             &                       &                     &                     \\
\bottomrule
\end{tabular}
}
\end{adjustwidth}
\label{tab:conversion}
% \vspace{-5pt}
\end{table}

% \resizebox{\textwidth}{!}{
% \begin{tabular}{c|ccc|cc|cc|c|c}
% \toprule
% \multirow{2}{*}{\makecell{\textbf{Data}}} & \multicolumn{3}{c|}{\textbf{CSR -> CSC}} & \multicolumn{2}{c|}{\textbf{COO -> DIA}}  & \multicolumn{2}{c|}{\textbf{DCSR -> ELL}} &  \textbf{DCSC -> BCSR} & \textbf{CSB -> DIA-variant} \\
% \cmidrule{2-10} 
%  & \IRName & \makecell{SparseTensor} & TACO & \IRName & TACO & \IRName & TACO & \IRName & \IRName  \\\hline
%  wv & 1 (0.002) & 1.01   & 37.20 & 1 (0.104) & 0.86 & 1 (0.883) &  & 1 (0.019) & 1 (0.065) \\
%  ee & 1 (0.000) & 2.58   & 11.17 & 1 (0.004) & 1.14 & 1 (0.020) &  & 1 (0.003) & 1 (0.004) \\
%  nm & 1 (0.009) & 2.90   & 0.62  & 1 (0.004) & 1.95 & 1 (0.034) &  & 1 (0.038) & 1 (0.030) \\
%  cm & 1 (0.003) & 1.65   & 0.32  & 1 (0.001) & 1.12 & 1 (0.009) &  & 1 (0.014) & 1 (0.009) \\
%  ct & 1 (0.043) & 1.79   & 0.72  & 1 (0.018) & 1.88 & 1 (0.170) &  & 1 (0.151) & 1 (0.169) \\
%  lp & 1 (0.672) & 0.98   & 0.56  & 1 (0.430) & 0.96 & 1 (4.103) &  & 1 (2.634) & 1 (4.352) \\
%  tp & 1 (0.467) & 1.19   & 0.27  & 1 (0.148) & 0.93 & 1 (1.619) &  & 1 (2.335) & 1 (5.584) \\
%  ts & 1 (0.534) & 0.85   & 0.31  & 1 (0.185) & 1.01 & 1 (4.768) &  & 1 (1.651) & 1 (2.319) \\
%  ch & 1 (0.005) & 1.01   & 0.17  & 1 (0.001) & 0.98 & 1 (0.009) &  & 1 (0.017) & 1 (0.012) \\
%  mj & 1 (0.033) & 1.25   & 0.27  & 1 (0.011) & 0.91 & 1 (0.082) &  & 1 (0.130) & 1 (0.153) \\
%  sh & 1 (0.006) & 1.35   & 0.30  & 1 (0.002) & 0.84 & 1 (0.022) &  & 1 (0.023) & 1 (0.017) \\
%  bm & 1 (0.014) & 1.27   & 0.21  & 1 (0.004) & 0.67 & 1 (0.033) &  & 1 (0.054) & 1 (0.060) \\\midrule
%  GM & 1         & 1.80   & 0.67  & 1         & 1.17 & 1         &  & 1         & 1         \\
% \bottomrule
% \end{tabular}
% }

% The format DIA-V is a short name of the DIA-variant format. Empty cells (`-') are due to segmentation fault errors of the generated conversion code. 
% \resizebox{\textwidth}{!}{
% \begin{tabular}{c|ccc|ccc|cc|c|c}
% \toprule
% \multirow{2}{*}{\makecell{\textbf{Data}}} & \multicolumn{3}{c|}{\textbf{CSR -> CSC}} & \multicolumn{3}{c|}{\textbf{COO -> DIA}}  & \multicolumn{2}{c|}{\textbf{DCSR -> ELL}} &  \textbf{DCSC -> BCSR} & \textbf{CSB -> DIA-V} \\
% \cmidrule{2-11} 
%  & \IRName & \makecell{MLIR\\SparseTensor} & TACO & \makecell{\IRName\\w/ fusion} & \makecell{\IRName\\w/o fusion} & TACO & \IRName & TACO & \IRName & \IRName  \\\hline
%  wv & 1 (0.002) & 1.01   & 37.20 & 1 (0.104) & 0.78 & 0.86 & 1 (0.883) & & (0.019) & (0.065) \\
%  ee & 1 (0.000) & 2.58  & 11.17 & 1 (0.004) & 0.93 & 1.14 & 1 (0.020) & & (0.003) & (0.004) \\
%  nm & 1 (0.009) & 2.90   & 0.62  & 1 (0.004) & 3.05 & 1.95 & 1 (0.034) & & (0.038) & (0.030) \\
%  cm & 1 (0.003) & 1.65   & 0.32  & 1 (0.001) & 2.91 & 1.12 & 1 (0.009) & & (0.014) & (0.009) \\
%  ct & 1 (0.043) & 1.79   & 0.72  & 1 (0.018) & 3.11 & 1.88 & 1 (0.170) & & (0.151) & (0.169) \\
%  lp & 1 (0.672) & 0.98   & 0.56  & 1 (0.430) & 2.69 & 0.96 & 1 (4.103) & & (2.634) & (4.352) \\
%  tp & 1 (0.467) & 1.19   & 0.27  & 1 (0.148) & 5.02 & 0.93 & 1 (1.619) & & (2.335) & (5.584) \\
%  ts & 1 (0.534) & 0.85   & 0.31  & 1 (0.185) & 3.11 & 1.01 & 1 (4.768) & & (1.651) & (2.319) \\
%  ch & 1 (0.005) & 1.01   & 0.17  & 1 (0.001) & 5.27 & 0.98 & 1 (0.009) & & (0.017) & (0.012) \\
%  mj & 1 (0.033) & 1.25   & 0.27  & 1 (0.011) & 3.31 & 0.91 & 1 (0.082) & & (0.130) & (0.153) \\
%  sh & 1 (0.006) & 1.35   & 0.30  & 1 (0.002) & 3.05 & 0.84 & 1 (0.022) & & (0.023) & (0.017) \\
%  bm & 1 (0.014) & 1.27   & 0.21  & 1 (0.004) & 2.99 & 0.67 & 1 (0.033) & & (0.054) & (0.060) \\\midrule
%  GM & 1         & 1.80   & 0.67  & 1         & 2.32 & 1.17 & 1         & &         &         \\
% \bottomrule
% \end{tabular}
% }

% \begin{tabular}{c|ccc|c|c|ccc|c|c}
% \toprule
% \multirow{2}{*}{\makecell{\textbf{Data}}} & \multicolumn{3}{c|}{\textbf{CSR -> CSC}} & \textbf{COO -> BDIA} & \multirow{2}{*}{\makecell{\textbf{Data}}} & \multicolumn{3}{c|}{\textbf{COO -> DIA}}  & \multirow{2}{*}{\makecell{\textbf{Data}}} &  \textbf{COO -> BELL}  \\
% \cmidrule{2-4} \cmidrule{5-5} \cmidrule{7-9} \cmidrule{11-11} 
%  & \IRName & \makecell{MLIR\\SparseTensor} & TACO & \IRName & & \makecell{\IRName\\w/ fusion} & \makecell{\IRName\\w/o fusion} & TACO &  & \IRName  \\\hline
%  ge & 1(2.512) & 1.14(2.867) &  & (8.946) & wv & 1(0.104) & 0.78(0.081) & 0.81(0.084) & c8 & (0.118) \\
%  ss & 1(0.863) & 1.24(1.073) &  & (1.203) & ee & 1(0.004) & 0.93(0.004) & 1.40(0.006) & ee & (0.001) \\
%  ra & 1(0.573) & 1.08(0.617) &  & (0.733) & nm & 1(0.004) & 3.05(0.013) & 2.07(0.009) & nm & (0.060) \\
%  mc & 1(0.393) & 1.18(0.464) &  & ()      & cm & 1(0.001) & 2.91(0.003) & 1.09(0.001) & h1 & (0.074) \\
%  vs & 1(1.137) & 1.11(1.262) &  & (0.660) & ct & 1(0.018) & 3.11(0.055) & 1.91(0.034) & b9 & (0.089) \\
%  lp & 1(0.619) & 1.09(0.674) &  & (2.082) & lp & 1(0.430) & 2.69(1.156) & 0.89(0.382) & cr & (0.008) \\
%  tp & 1(0.487) & 1.19(0.582) &  & (2.090) & tp & 1(0.148) & 5.02(0.744) & 0.82(0.122) & tf-0.6 & (0.339) \\
%  ts & 1(0.562) & 0.83(0.466) &  & (1.359) & ts & 1(0.185) & 3.11(0.576) & 0.89(0.165) & tf-0.7 & (0.274) \\
% \bottomrule
% \end{tabular}

% \resizebox{0.48\textwidth}{!}{
% \begin{tabular}{c|ccc|c}
% \toprule
% \multirow{2}{*}{\textbf{Data}} & \multicolumn{3}{c|}{\textbf{CSR -> CSC}} & \textbf{COO -> BELL} \\
% \cmidrule{2-4} \cmidrule{5-5}  
%  & \IRName & \makecell{MLIR\\{SparseTensor}} & {TACO} & \IRName \\\hline
% % wv &  &  &  & 1(0.104) & 0.78(0.081) & 0.81(0.084) &  &  \\
% % ee &  &  &  & 1(0.004) & 0.93(0.004) & 1.40(0.006) &  &  \\
% % nm &  &  &  & 1(0.004) & 3.05(0.013) & 2.07(0.009) &  &  \\
% % cm &  &  &  & 1(0.001) & 2.91(0.003) & 1.09(0.001) &  &  \\
% % ct &  &  &  & 1(0.018) & 3.11(0.055) & 1.91(0.034) &  &  \\
% % lp &  &  &  & 1(0.430) & 2.69(1.156) & 0.89(0.382) &  &  \\
% % tp &  &  &  & 1(0.148) & 5.02(0.744) & 0.82(0.122) &  &  \\
% % ts &  &  &  & 1(0.185) & 3.11(0.576) & 0.89(0.165) &  &  \\
% % \cline{2-3}
% %                                              & \lstinline|relayout(lv)| & Rearrange the storage of subtensors specified by level \lstinline|lv| into specific memory spaces\\
% \bottomrule
% \end{tabular}
% }
% \resizebox{0.32\textwidth}{!}{
% \begin{tabular}{c|ccc}
% \toprule
% \multirow{2}{*}{\textbf{Data}} & \multicolumn{3}{c}{\textbf{COO -> DIA}} \\
% \cmidrule{2-4} 
%  & \IRName & \makecell{\IRName\\w/o fusion} & TACO \\\hline

% % \cline{2-3}
% %                                              & \lstinline|relayout(lv)| & Rearrange the storage of subtensors specified by level \lstinline|lv| into specific memory spaces\\
% \bottomrule
% \end{tabular}
% }
% \resizebox{0.19\textwidth}{!}{
% \begin{tabular}{c|c}
% \toprule
% \multirow{2}{*}{\textbf{Data}} & \multicolumn{1}{c}{\textbf{COO -> BDIA}} \\
% \cmidrule{2-2} 
%  & \IRName \\\hline

% % \cline{2-3}
% %                                              & \lstinline|relayout(lv)| & Rearrange the storage of subtensors specified by level \lstinline|lv| into specific memory spaces\\
% \bottomrule
% \end{tabular}
% }

% \resizebox{0.69\textwidth}{!}{
% \begin{tabular}{c|ccc|ccc|c|c}
% \toprule
% \multirow{2}{*}{\lstinline{DS}} & \multicolumn{3}{c|}{\lstinline{CSR -> CSC}} & \multicolumn{3}{c|}{\lstinline{COO -> DIA}} & \lstinline{COO -> BDIA} & \lstinline{COO -> BELL} \\
% \cmidrule{2-4} \cmidrule{5-7} \cmidrule{8-8} \cmidrule{9-9} 
%  & \IRName & \makecell{MLIR\\SparseTensor} & TACO & \IRName & \makecell{\IRName\\w/o fusion} & TACO & \IRName & \IRName \\\hline
% wv &  &  &  & 1(0.104) & 0.78(0.081) & 0.81(0.084) &  &  \\
% ee &  &  &  & 1(0.004) & 0.93(0.004) & 1.40(0.006) &  &  \\
% nm &  &  &  & 1(0.004) & 3.05(0.013) & 2.07(0.009) &  &  \\
% cm &  &  &  & 1(0.001) & 2.91(0.003) & 1.09(0.001) &  &  \\
% ct &  &  &  & 1(0.018) & 3.11(0.055) & 1.91(0.034) &  &  \\
% lp &  &  &  & 1(0.430) & 2.69(1.156) & 0.89(0.382) &  &  \\
% tp &  &  &  & 1(0.148) & 5.02(0.744) & 0.82(0.122) &  &  \\
% ts &  &  &  & 1(0.185) & 3.11(0.576) & 0.89(0.165) &  &  \\
% % \cline{2-3}
% %                                              & \lstinline|relayout(lv)| & Rearrange the storage of subtensors specified by level \lstinline|lv| into specific memory spaces\\
% \bottomrule
% \end{tabular}
% }

% \multirow{2}{*}{\lstinline{Data}} & \multicolumn{3}{c|}{\lstinline{CSR -> CSC}} & \lstinline{COO -> BELL} \\
% \cmidrule{2-4} \cmidrule{5-5}  
%  & \lstinline{UniSparse} & \makecell{\lstinline{MLIR}\\\lstinline{SparseTensor}} & \lstinline{TACO} & \lstinline{UniSparse} \\\hline
 

==> figs-tabs/tab-conversion-stdv.tex <==
\begin{table}[ht]%[tb!]
\centering
% \vspace{-5pt}
\caption{
Comparison of normalized execution times for format conversion programs generated by \IRName, MLIR SparseTensor dialect, and \rev{the format conversion artifact of} TACO~\cite{github_chou2020automatic}, relative to the performance achieved by \IRName. The actual execution times (in \textit{seconds}) for format conversion programs generated by \IRName are shown in parentheses. 
}
% \vspace{-5pt}
\footnotesize
\setlength\tabcolsep{5pt} % Reduce the white space margins in each cell
\lstset{%
tabsize=2,
columns=fullflexible,
basicstyle=\ttfamily\scriptsize,
breaklines=true,
breakatwhitespace,
escapeinside={(*}{*)},
alsoletter={\., \_},
morekeywords={tile\_division, tile\_union, enumerate, reorder, schedule, move\_lv, trim, fill, merge, split, vectorize, devectorize, pad, pack, partition}
}
\resizebox{0.85\textwidth}{!}{\tablerev
\begin{tabular}{c|ccc|cc|cc}
\toprule
\multirow{2}{*}{\makecell{\textbf{Data}}} & \multicolumn{3}{c|}{\textbf{CSR} $\rightarrow$ \textbf{CSC}} & \multicolumn{2}{c|}{\textbf{COO} $\rightarrow$ \textbf{DIA}}  & \multicolumn{2}{c}{\textbf{COO} $\rightarrow$ \textbf{ELL}} \\
\cmidrule{2-8} 
    & \IRName & \makecell{SparseTensor} & TACO & \IRName & TACO & \IRName & TACO  \\\midrule
 wv & 1 (0.001 $\pm$ 0.000) &  3.962 $\pm$ 0.391 & 1.448 $\pm$ 0.055 & 1 (0.065 $\pm$ 0.004) & 1.404 $\pm$ 0.013 & 1 (0.014 $\pm$ 0.001) & 1.19  \\
 ee & 1 (0.000 $\pm$ 0.000) &  5.075 $\pm$ 0.660 & 1.259 $\pm$ 0.065 & 1 (0.003 $\pm$ 0.000) & 1.609 $\pm$ 0.066 & 1 (0.001 $\pm$ 0.000) & 1.23  \\
 nm & 1 (0.002 $\pm$ 0.000) & 14.594 $\pm$ 0.366 & 2.474 $\pm$ 0.030 & 1 (0.003 $\pm$ 0.000) & 2.394 $\pm$ 0.025 & 1 (0.006 $\pm$ 0.000) & 1.70  \\
 cm & 1 (0.001 $\pm$ 0.000) & 10.042 $\pm$ 0.559 & 1.828 $\pm$ 0.021 & 1 (0.001 $\pm$ 0.000) & 1.631 $\pm$ 0.020 & 1 (0.002 $\pm$ 0.000) & 1.44  \\
 ct & 1 (0.009 $\pm$ 0.000) &  8.955 $\pm$ 0.449 & 2.012 $\pm$ 0.014 & 1 (0.013 $\pm$ 0.000) & 2.356 $\pm$ 0.032 & 1 (0.023 $\pm$ 0.000) & 1.97  \\
 lp & 1 (0.193 $\pm$ 0.003) &  3.416 $\pm$ 0.025 & 0.991 $\pm$ 0.021 & 1 (0.352 $\pm$ 0.008) & 1.231 $\pm$ 0.012 & 1 (0.298 $\pm$ 0.005) & 1.22  \\
 tp & 1 (0.139 $\pm$ 0.002) &  4.039 $\pm$ 0.032 & 1.205 $\pm$ 0.025 & 1 (0.127 $\pm$ 0.002) & 1.043 $\pm$ 0.025 & 1 (0.220 $\pm$ 0.002) & 0.91  \\
 ts & 1 (0.168 $\pm$ 0.001) &  2.747 $\pm$ 0.034 & 0.966 $\pm$ 0.013 & 1 (0.163 $\pm$ 0.002) & 1.176 $\pm$ 0.011 & 1 (0.249 $\pm$ 0.004) & 1.10  \\
 ch & 1 (0.001 $\pm$ 0.000) &  6.253 $\pm$ 0.067 & 0.637 $\pm$ 0.017 & 1 (0.001 $\pm$ 0.000) & 0.974 $\pm$ 0.019 & 1 (0.002 $\pm$ 0.000) & 0.53  \\
 mj & 1 (0.008 $\pm$ 0.000) &  5.148 $\pm$ 0.072 & 0.748 $\pm$ 0.006 & 1 (0.008 $\pm$ 0.000) & 1.221 $\pm$ 0.015 & 1 (0.017 $\pm$ 0.000) & 0.58  \\
 sh & 1 (0.001 $\pm$ 0.000) &  5.871 $\pm$ 0.667 & 0.637 $\pm$ 0.009 & 1 (0.001 $\pm$ 0.000) & 1.434 $\pm$ 0.019 & 1 (0.003 $\pm$ 0.000) & 0.72  \\
 bm & 1 (0.003 $\pm$ 0.000) &  6.025 $\pm$ 0.110 & 0.753 $\pm$ 0.006 & 1 (0.004 $\pm$ 0.000) & 0.813 $\pm$ 0.007 & 1 (0.007 $\pm$ 0.000) & 1.28  \\\midrule
 Geomean & 1                &  5.685             & 1.131             & 1                     & 1.369             & 1         & 1.08  \\
\bottomrule
\end{tabular}
}
\resizebox{0.68\textwidth}{!}{
% \relscale{0.5}
% \fontsize{3pt}{1pt}\selectfont
% \setlength\tabcolsep{3pt} % Reduce the white space margins in each cell
\begin{tabular}{c|c|c|c|c}
% \toprule
\multirow{2}{*}{\makecell{\textbf{Data}}} & \textbf{DCSC} $\rightarrow$ \textbf{BCSR} & \textbf{CSB} $\rightarrow$ \textbf{DIA-variant} & \textbf{COO} $\rightarrow$ \textbf{C\textsuperscript{2}SR} & \textbf{COO} $\rightarrow$ \textbf{CISR}\\
\cmidrule{2-5} 
    & \IRName & \IRName & \IRName & \IRName \\\midrule
 wv & (0.012 $\pm$ 0.001) & (0.067 $\pm$ 0.001) & (0.003 $\pm$ 0.000) & (0.003 $\pm$ 0.000) \\
 ee & (0.003 $\pm$ 0.000) & (0.004 $\pm$ 0.000) & (0.001 $\pm$ 0.000) & (0.001 $\pm$ 0.000) \\
 nm & (0.039 $\pm$ 0.000) & (0.032 $\pm$ 0.001) & (0.017 $\pm$ 0.000) & (0.017 $\pm$ 0.000) \\
 cm & (0.012 $\pm$ 0.001) & (0.007 $\pm$ 0.000) & (0.005 $\pm$ 0.000) & (0.005 $\pm$ 0.000) \\
 ct & (0.148 $\pm$ 0.001) & (0.184 $\pm$ 0.002) & (0.071 $\pm$ 0.001) & (0.077 $\pm$ 0.001) \\
 lp & (2.554 $\pm$ 0.015) & (4.509 $\pm$ 0.031) & (1.069 $\pm$ 0.004) & (1.080 $\pm$ 0.021) \\
 tp & (2.249 $\pm$ 0.010) & (6.157 $\pm$ 0.038) & (0.929 $\pm$ 0.009) & (1.303 $\pm$ 0.062) \\
 ts & (1.733 $\pm$ 0.009) & (2.509 $\pm$ 0.017) & (0.541 $\pm$ 0.005) & (0.508 $\pm$ 0.045) \\
 ch & (0.015 $\pm$ 0.001) & (0.009 $\pm$ 0.000) & (0.006 $\pm$ 0.001) & (0.007 $\pm$ 0.001) \\
 mj & (0.134 $\pm$ 0.001) & (0.178 $\pm$ 0.002) & (0.060 $\pm$ 0.001) & (0.072 $\pm$ 0.001) \\
 sh & (0.023 $\pm$ 0.000) & (0.018 $\pm$ 0.000) & (0.011 $\pm$ 0.000) & (0.013 $\pm$ 0.000) \\
 bm & (0.058 $\pm$ 0.001) & (0.063 $\pm$ 0.001) & (0.026 $\pm$ 0.000) & (0.031 $\pm$ 0.000) \\
 % Geomean & 1    & 5.79   & 1.21  & 1         & 1.21 & 1         & 1.08 &         &         &         &    \\
\bottomrule
\end{tabular}
}
\label{tab:conversion}
% \vspace{-5pt}
\end{table}

% \resizebox{\textwidth}{!}{
% \begin{tabular}{c|ccc|cc|cc|c|c}
% \toprule
% \multirow{2}{*}{\makecell{\textbf{Data}}} & \multicolumn{3}{c|}{\textbf{CSR -> CSC}} & \multicolumn{2}{c|}{\textbf{COO -> DIA}}  & \multicolumn{2}{c|}{\textbf{DCSR -> ELL}} &  \textbf{DCSC -> BCSR} & \textbf{CSB -> DIA-variant} \\
% \cmidrule{2-10} 
%  & \IRName & \makecell{SparseTensor} & TACO & \IRName & TACO & \IRName & TACO & \IRName & \IRName  \\\hline
%  wv & 1 (0.002) & 1.01   & 37.20 & 1 (0.104) & 0.86 & 1 (0.883) &  & 1 (0.019) & 1 (0.065) \\
%  ee & 1 (0.000) & 2.58   & 11.17 & 1 (0.004) & 1.14 & 1 (0.020) &  & 1 (0.003) & 1 (0.004) \\
%  nm & 1 (0.009) & 2.90   & 0.62  & 1 (0.004) & 1.95 & 1 (0.034) &  & 1 (0.038) & 1 (0.030) \\
%  cm & 1 (0.003) & 1.65   & 0.32  & 1 (0.001) & 1.12 & 1 (0.009) &  & 1 (0.014) & 1 (0.009) \\
%  ct & 1 (0.043) & 1.79   & 0.72  & 1 (0.018) & 1.88 & 1 (0.170) &  & 1 (0.151) & 1 (0.169) \\
%  lp & 1 (0.672) & 0.98   & 0.56  & 1 (0.430) & 0.96 & 1 (4.103) &  & 1 (2.634) & 1 (4.352) \\
%  tp & 1 (0.467) & 1.19   & 0.27  & 1 (0.148) & 0.93 & 1 (1.619) &  & 1 (2.335) & 1 (5.584) \\
%  ts & 1 (0.534) & 0.85   & 0.31  & 1 (0.185) & 1.01 & 1 (4.768) &  & 1 (1.651) & 1 (2.319) \\
%  ch & 1 (0.005) & 1.01   & 0.17  & 1 (0.001) & 0.98 & 1 (0.009) &  & 1 (0.017) & 1 (0.012) \\
%  mj & 1 (0.033) & 1.25   & 0.27  & 1 (0.011) & 0.91 & 1 (0.082) &  & 1 (0.130) & 1 (0.153) \\
%  sh & 1 (0.006) & 1.35   & 0.30  & 1 (0.002) & 0.84 & 1 (0.022) &  & 1 (0.023) & 1 (0.017) \\
%  bm & 1 (0.014) & 1.27   & 0.21  & 1 (0.004) & 0.67 & 1 (0.033) &  & 1 (0.054) & 1 (0.060) \\\midrule
%  GM & 1         & 1.80   & 0.67  & 1         & 1.17 & 1         &  & 1         & 1         \\
% \bottomrule
% \end{tabular}
% }

% The format DIA-V is a short name of the DIA-variant format. Empty cells (`-') are due to segmentation fault errors of the generated conversion code. 
% \resizebox{\textwidth}{!}{
% \begin{tabular}{c|ccc|ccc|cc|c|c}
% \toprule
% \multirow{2}{*}{\makecell{\textbf{Data}}} & \multicolumn{3}{c|}{\textbf{CSR -> CSC}} & \multicolumn{3}{c|}{\textbf{COO -> DIA}}  & \multicolumn{2}{c|}{\textbf{DCSR -> ELL}} &  \textbf{DCSC -> BCSR} & \textbf{CSB -> DIA-V} \\
% \cmidrule{2-11} 
%  & \IRName & \makecell{MLIR\\SparseTensor} & TACO & \makecell{\IRName\\w/ fusion} & \makecell{\IRName\\w/o fusion} & TACO & \IRName & TACO & \IRName & \IRName  \\\hline
%  wv & 1 (0.002) & 1.01   & 37.20 & 1 (0.104) & 0.78 & 0.86 & 1 (0.883) & & (0.019) & (0.065) \\
%  ee & 1 (0.000) & 2.58  & 11.17 & 1 (0.004) & 0.93 & 1.14 & 1 (0.020) & & (0.003) & (0.004) \\
%  nm & 1 (0.009) & 2.90   & 0.62  & 1 (0.004) & 3.05 & 1.95 & 1 (0.034) & & (0.038) & (0.030) \\
%  cm & 1 (0.003) & 1.65   & 0.32  & 1 (0.001) & 2.91 & 1.12 & 1 (0.009) & & (0.014) & (0.009) \\
%  ct & 1 (0.043) & 1.79   & 0.72  & 1 (0.018) & 3.11 & 1.88 & 1 (0.170) & & (0.151) & (0.169) \\
%  lp & 1 (0.672) & 0.98   & 0.56  & 1 (0.430) & 2.69 & 0.96 & 1 (4.103) & & (2.634) & (4.352) \\
%  tp & 1 (0.467) & 1.19   & 0.27  & 1 (0.148) & 5.02 & 0.93 & 1 (1.619) & & (2.335) & (5.584) \\
%  ts & 1 (0.534) & 0.85   & 0.31  & 1 (0.185) & 3.11 & 1.01 & 1 (4.768) & & (1.651) & (2.319) \\
%  ch & 1 (0.005) & 1.01   & 0.17  & 1 (0.001) & 5.27 & 0.98 & 1 (0.009) & & (0.017) & (0.012) \\
%  mj & 1 (0.033) & 1.25   & 0.27  & 1 (0.011) & 3.31 & 0.91 & 1 (0.082) & & (0.130) & (0.153) \\
%  sh & 1 (0.006) & 1.35   & 0.30  & 1 (0.002) & 3.05 & 0.84 & 1 (0.022) & & (0.023) & (0.017) \\
%  bm & 1 (0.014) & 1.27   & 0.21  & 1 (0.004) & 2.99 & 0.67 & 1 (0.033) & & (0.054) & (0.060) \\\midrule
%  GM & 1         & 1.80   & 0.67  & 1         & 2.32 & 1.17 & 1         & &         &         \\
% \bottomrule
% \end{tabular}
% }

% \begin{tabular}{c|ccc|c|c|ccc|c|c}
% \toprule
% \multirow{2}{*}{\makecell{\textbf{Data}}} & \multicolumn{3}{c|}{\textbf{CSR -> CSC}} & \textbf{COO -> BDIA} & \multirow{2}{*}{\makecell{\textbf{Data}}} & \multicolumn{3}{c|}{\textbf{COO -> DIA}}  & \multirow{2}{*}{\makecell{\textbf{Data}}} &  \textbf{COO -> BELL}  \\
% \cmidrule{2-4} \cmidrule{5-5} \cmidrule{7-9} \cmidrule{11-11} 
%  & \IRName & \makecell{MLIR\\SparseTensor} & TACO & \IRName & & \makecell{\IRName\\w/ fusion} & \makecell{\IRName\\w/o fusion} & TACO &  & \IRName  \\\hline
%  ge & 1(2.512) & 1.14(2.867) &  & (8.946) & wv & 1(0.104) & 0.78(0.081) & 0.81(0.084) & c8 & (0.118) \\
%  ss & 1(0.863) & 1.24(1.073) &  & (1.203) & ee & 1(0.004) & 0.93(0.004) & 1.40(0.006) & ee & (0.001) \\
%  ra & 1(0.573) & 1.08(0.617) &  & (0.733) & nm & 1(0.004) & 3.05(0.013) & 2.07(0.009) & nm & (0.060) \\
%  mc & 1(0.393) & 1.18(0.464) &  & ()      & cm & 1(0.001) & 2.91(0.003) & 1.09(0.001) & h1 & (0.074) \\
%  vs & 1(1.137) & 1.11(1.262) &  & (0.660) & ct & 1(0.018) & 3.11(0.055) & 1.91(0.034) & b9 & (0.089) \\
%  lp & 1(0.619) & 1.09(0.674) &  & (2.082) & lp & 1(0.430) & 2.69(1.156) & 0.89(0.382) & cr & (0.008) \\
%  tp & 1(0.487) & 1.19(0.582) &  & (2.090) & tp & 1(0.148) & 5.02(0.744) & 0.82(0.122) & tf-0.6 & (0.339) \\
%  ts & 1(0.562) & 0.83(0.466) &  & (1.359) & ts & 1(0.185) & 3.11(0.576) & 0.89(0.165) & tf-0.7 & (0.274) \\
% \bottomrule
% \end{tabular}

% \resizebox{0.48\textwidth}{!}{
% \begin{tabular}{c|ccc|c}
% \toprule
% \multirow{2}{*}{\textbf{Data}} & \multicolumn{3}{c|}{\textbf{CSR -> CSC}} & \textbf{COO -> BELL} \\
% \cmidrule{2-4} \cmidrule{5-5}  
%  & \IRName & \makecell{MLIR\\{SparseTensor}} & {TACO} & \IRName \\\hline
% % wv &  &  &  & 1(0.104) & 0.78(0.081) & 0.81(0.084) &  &  \\
% % ee &  &  &  & 1(0.004) & 0.93(0.004) & 1.40(0.006) &  &  \\
% % nm &  &  &  & 1(0.004) & 3.05(0.013) & 2.07(0.009) &  &  \\
% % cm &  &  &  & 1(0.001) & 2.91(0.003) & 1.09(0.001) &  &  \\
% % ct &  &  &  & 1(0.018) & 3.11(0.055) & 1.91(0.034) &  &  \\
% % lp &  &  &  & 1(0.430) & 2.69(1.156) & 0.89(0.382) &  &  \\
% % tp &  &  &  & 1(0.148) & 5.02(0.744) & 0.82(0.122) &  &  \\
% % ts &  &  &  & 1(0.185) & 3.11(0.576) & 0.89(0.165) &  &  \\
% % \cline{2-3}
% %                                              & \lstinline|relayout(lv)| & Rearrange the storage of subtensors specified by level \lstinline|lv| into specific memory spaces\\
% \bottomrule
% \end{tabular}
% }
% \resizebox{0.32\textwidth}{!}{
% \begin{tabular}{c|ccc}
% \toprule
% \multirow{2}{*}{\textbf{Data}} & \multicolumn{3}{c}{\textbf{COO -> DIA}} \\
% \cmidrule{2-4} 
%  & \IRName & \makecell{\IRName\\w/o fusion} & TACO \\\hline

% % \cline{2-3}
% %                                              & \lstinline|relayout(lv)| & Rearrange the storage of subtensors specified by level \lstinline|lv| into specific memory spaces\\
% \bottomrule
% \end{tabular}
% }
% \resizebox{0.19\textwidth}{!}{
% \begin{tabular}{c|c}
% \toprule
% \multirow{2}{*}{\textbf{Data}} & \multicolumn{1}{c}{\textbf{COO -> BDIA}} \\
% \cmidrule{2-2} 
%  & \IRName \\\hline

% % \cline{2-3}
% %                                              & \lstinline|relayout(lv)| & Rearrange the storage of subtensors specified by level \lstinline|lv| into specific memory spaces\\
% \bottomrule
% \end{tabular}
% }

% \resizebox{0.69\textwidth}{!}{
% \begin{tabular}{c|ccc|ccc|c|c}
% \toprule
% \multirow{2}{*}{\lstinline{DS}} & \multicolumn{3}{c|}{\lstinline{CSR -> CSC}} & \multicolumn{3}{c|}{\lstinline{COO -> DIA}} & \lstinline{COO -> BDIA} & \lstinline{COO -> BELL} \\
% \cmidrule{2-4} \cmidrule{5-7} \cmidrule{8-8} \cmidrule{9-9} 
%  & \IRName & \makecell{MLIR\\SparseTensor} & TACO & \IRName & \makecell{\IRName\\w/o fusion} & TACO & \IRName & \IRName \\\hline
% wv &  &  &  & 1(0.104) & 0.78(0.081) & 0.81(0.084) &  &  \\
% ee &  &  &  & 1(0.004) & 0.93(0.004) & 1.40(0.006) &  &  \\
% nm &  &  &  & 1(0.004) & 3.05(0.013) & 2.07(0.009) &  &  \\
% cm &  &  &  & 1(0.001) & 2.91(0.003) & 1.09(0.001) &  &  \\
% ct &  &  &  & 1(0.018) & 3.11(0.055) & 1.91(0.034) &  &  \\
% lp &  &  &  & 1(0.430) & 2.69(1.156) & 0.89(0.382) &  &  \\
% tp &  &  &  & 1(0.148) & 5.02(0.744) & 0.82(0.122) &  &  \\
% ts &  &  &  & 1(0.185) & 3.11(0.576) & 0.89(0.165) &  &  \\
% % \cline{2-3}
% %                                              & \lstinline|relayout(lv)| & Rearrange the storage of subtensors specified by level \lstinline|lv| into specific memory spaces\\
% \bottomrule
% \end{tabular}
% }

% \multirow{2}{*}{\lstinline{Data}} & \multicolumn{3}{c|}{\lstinline{CSR -> CSC}} & \lstinline{COO -> BELL} \\
% \cmidrule{2-4} \cmidrule{5-5}  
%  & \lstinline{UniSparse} & \makecell{\lstinline{MLIR}\\\lstinline{SparseTensor}} & \lstinline{TACO} & \lstinline{UniSparse} \\\hline
 

==> figs-tabs/tab-conversion.tex <==
\begin{table}[ht]%[tb!]
\centering
% \vspace{-5pt}
\caption{
Comparison of normalized execution times for format conversion programs generated by \IRName, MLIR SparseTensor dialect, and \rev{the format conversion artifact of} TACO~\cite{github_chou2020automatic}, relative to the performance achieved by \IRName. The actual execution times (in \textit{seconds}) for format conversion programs generated by \IRName are shown in parentheses. 
% This table excludes cases not supported by the compiler frameworks, such as COO $\rightarrow$ DIA and COO $\rightarrow$ ELL in MLIR SparseTensor, as well as DCSC $\rightarrow$ BCSR, CSB $\rightarrow$ DIA-variant, COO $\rightarrow$ C\textsuperscript{2}SR, and COO $\rightarrow$ CISR in both TACO and MLIR SparseTensor.
% Normalized execution time comparison of format conversion programs generated by \IRName, MLIR SparseTensor dialect, and TACO, relative to the performance that \IRName achieves. The actual execution times (in \textbf{seconds}) of the format conversion programs generated by \IRName are shown in parentheses. Missing columns are cases not supported by the compiler frameworks, such as DCSC->BCSR and CSB -> DIA-variant in TACO and MLIR SparseTensor, are not shown in this table.
}
% \vspace{-5pt}
\footnotesize
\setlength\tabcolsep{5pt} % Reduce the white space margins in each cell
\lstset{%
tabsize=2,
columns=fullflexible,
basicstyle=\ttfamily\scriptsize,
breaklines=true,
breakatwhitespace,
escapeinside={(*}{*)},
alsoletter={\., \_},
morekeywords={tile\_division, tile\_union, enumerate, reorder, schedule, move\_lv, trim, fill, merge, split, vectorize, devectorize, pad, pack, partition}
}
\resizebox{\textwidth}{!}{\tablerev
\begin{tabular}{c|ccc|cc|cc|c|c|c|c}
\toprule
\multirow{2}{*}{\makecell{\textbf{Data}}} & \multicolumn{3}{c|}{\textbf{CSR} $\rightarrow$ \textbf{CSC}} & \multicolumn{2}{c|}{\textbf{COO} $\rightarrow$ \textbf{DIA}}  & \multicolumn{2}{c|}{\textbf{COO} $\rightarrow$ \textbf{ELL}} & \textbf{DCSC} $\rightarrow$ \textbf{BCSR} & \textbf{CSB} $\rightarrow$ \textbf{DIA-variant} & \textbf{COO} $\rightarrow$ \textbf{C\textsuperscript{2}SR} & \textbf{COO} $\rightarrow$ \textbf{CISR}\\
\cmidrule{2-12} 
    & \IRName & \makecell{SparseTensor} & TACO & \IRName & TACO & \IRName & TACO & \IRName & \IRName & \IRName & \IRName \\\midrule
 wv & 1 (0.001) & 2.98   & 1.50  & 1 (0.080) & 1.11 & 1 (0.016) & 1.19 & (0.019) & (0.065) & (0.004) & (0.004) \\
 ee & 1 (0.000) & 11.18  & 3.00  & 1 (0.004) & 1.10 & 1 (0.001) & 1.23 & (0.003) & (0.004) & (0.001) & (0.001) \\
 nm & 1 (0.002) & 14.43  & 2.63  & 1 (0.004) & 2.16 & 1 (0.005) & 1.70 & (0.038) & (0.030) & (0.019) & (0.018) \\
 cm & 1 (0.001) & 8.16   & 1.71  & 1 (0.001) & 1.33 & 1 (0.002) & 1.44 & (0.014) & (0.009) & (0.006) & (0.007) \\
 ct & 1 (0.010) & 8.17   & 1.79  & 1 (0.014) & 2.40 & 1 (0.022) & 1.97 & (0.151) & (0.169) & (0.070) & (0.074) \\
 lp & 1 (0.185) & 3.56   & 0.92  & 1 (0.377) & 1.09 & 1 (0.270) & 1.22 & (2.634) & (4.352) & (1.106) & (1.114) \\
 tp & 1 (0.131) & 4.25   & 1.11  & 1 (0.139) & 0.99 & 1 (0.216) & 0.91 & (2.335) & (5.584) & (0.943) & (1.303) \\
 ts & 1 (0.152) & 3.00   & 0.97  & 1 (0.168) & 1.11 & 1 (0.230) & 1.10 & (1.651) & (2.319) & (0.558) & (0.523) \\
 ch & 1 (0.001) & 4.65   & 0.60  & 1 (0.001) & 0.89 & 1 (0.002) & 0.53 & (0.017) & (0.012) & (0.008) & (0.010) \\
 mj & 1 (0.008) & 5.47   & 0.76  & 1 (0.009) & 1.11 & 1 (0.016) & 0.58 & (0.130) & (0.153) & (0.057) & (0.068) \\
 sh & 1 (0.002) & 5.36   & 0.63  & 1 (0.002) & 1.19 & 1 (0.003) & 0.72 & (0.023) & (0.017) & (0.013) & (0.014) \\
 bm & 1 (0.003) & 7.10   & 0.92  & 1 (0.004) & 0.78 & 1 (0.003) & 1.28 & (0.054) & (0.060) & (0.025) & (0.031) \\\midrule
 Geomean & 1    & 5.79   & 1.21  & 1         & 1.21 & 1         & 1.08 &         &         &         &    \\
\bottomrule
\end{tabular}
% \begin{tabular}{c|ccc|cc|c|c|c|c}
% \toprule
% \multirow{2}{*}{\makecell{\textbf{Data}}} & \multicolumn{3}{c|}{\textbf{CSR -> CSC}} & \multicolumn{2}{c|}{\textbf{COO -> DIA}}  & \textbf{DCSC -> BCSR} & \textbf{CSB -> DIA-variant} & \textbf{COO -> C\textsuperscript{2}SR} & \textbf{COO -> CISR}\\
% \cmidrule{2-10} 
%  & \IRName & \makecell{SparseTensor} & TACO & \IRName & TACO & \IRName & \IRName & \IRName & \IRName \\\hline
%  wv & 1 (0.002) & 1.01   & 37.20 & 1 (0.104) & 0.86 & (0.019) & (0.065) & (0.004) & (0.004) \\
%  ee & 1 (0.000) & 2.58   & 11.17 & 1 (0.004) & 1.14 & (0.003) & (0.004) & (0.001) & (0.001) \\
%  nm & 1 (0.009) & 2.90   & 0.62  & 1 (0.004) & 1.95 & (0.038) & (0.030) & (0.019) & (0.018) \\
%  cm & 1 (0.003) & 1.65   & 0.32  & 1 (0.001) & 1.12 & (0.014) & (0.009) & (0.006) & (0.007) \\
%  ct & 1 (0.043) & 1.79   & 0.72  & 1 (0.018) & 1.88 & (0.151) & (0.169) & (0.070) & (0.074) \\
%  lp & 1 (0.672) & 0.98   & 0.56  & 1 (0.430) & 0.96 & (2.634) & (4.352) & (1.106) & (1.114) \\
%  tp & 1 (0.467) & 1.19   & 0.27  & 1 (0.148) & 0.93 & (2.335) & (5.584) & (0.943) & (1.303) \\
%  ts & 1 (0.534) & 0.85   & 0.31  & 1 (0.185) & 1.01 & (1.651) & (2.319) & (0.558) & (0.523) \\
%  ch & 1 (0.005) & 1.01   & 0.17  & 1 (0.001) & 0.98 & (0.017) & (0.012) & (0.008) & (0.010) \\
%  mj & 1 (0.033) & 1.25   & 0.27  & 1 (0.011) & 0.91 & (0.130) & (0.153) & (0.057) & (0.068) \\
%  sh & 1 (0.006) & 1.35   & 0.30  & 1 (0.002) & 0.84 & (0.023) & (0.017) & (0.013) & (0.014) \\
%  bm & 1 (0.014) & 1.27   & 0.21  & 1 (0.004) & 0.67 & (0.054) & (0.060) & (0.025) & (0.031) \\\midrule
%  Geomean & 1         & 1.80   & 0.67  & 1         & 1.17 &          &         &         &    \\
% \bottomrule
% \end{tabular}
}
\label{tab:conversion}
% \vspace{-5pt}
\end{table}

% \resizebox{\textwidth}{!}{
% \begin{tabular}{c|ccc|cc|cc|c|c}
% \toprule
% \multirow{2}{*}{\makecell{\textbf{Data}}} & \multicolumn{3}{c|}{\textbf{CSR -> CSC}} & \multicolumn{2}{c|}{\textbf{COO -> DIA}}  & \multicolumn{2}{c|}{\textbf{DCSR -> ELL}} &  \textbf{DCSC -> BCSR} & \textbf{CSB -> DIA-variant} \\
% \cmidrule{2-10} 
%  & \IRName & \makecell{SparseTensor} & TACO & \IRName & TACO & \IRName & TACO & \IRName & \IRName  \\\hline
%  wv & 1 (0.002) & 1.01   & 37.20 & 1 (0.104) & 0.86 & 1 (0.883) &  & 1 (0.019) & 1 (0.065) \\
%  ee & 1 (0.000) & 2.58   & 11.17 & 1 (0.004) & 1.14 & 1 (0.020) &  & 1 (0.003) & 1 (0.004) \\
%  nm & 1 (0.009) & 2.90   & 0.62  & 1 (0.004) & 1.95 & 1 (0.034) &  & 1 (0.038) & 1 (0.030) \\
%  cm & 1 (0.003) & 1.65   & 0.32  & 1 (0.001) & 1.12 & 1 (0.009) &  & 1 (0.014) & 1 (0.009) \\
%  ct & 1 (0.043) & 1.79   & 0.72  & 1 (0.018) & 1.88 & 1 (0.170) &  & 1 (0.151) & 1 (0.169) \\
%  lp & 1 (0.672) & 0.98   & 0.56  & 1 (0.430) & 0.96 & 1 (4.103) &  & 1 (2.634) & 1 (4.352) \\
%  tp & 1 (0.467) & 1.19   & 0.27  & 1 (0.148) & 0.93 & 1 (1.619) &  & 1 (2.335) & 1 (5.584) \\
%  ts & 1 (0.534) & 0.85   & 0.31  & 1 (0.185) & 1.01 & 1 (4.768) &  & 1 (1.651) & 1 (2.319) \\
%  ch & 1 (0.005) & 1.01   & 0.17  & 1 (0.001) & 0.98 & 1 (0.009) &  & 1 (0.017) & 1 (0.012) \\
%  mj & 1 (0.033) & 1.25   & 0.27  & 1 (0.011) & 0.91 & 1 (0.082) &  & 1 (0.130) & 1 (0.153) \\
%  sh & 1 (0.006) & 1.35   & 0.30  & 1 (0.002) & 0.84 & 1 (0.022) &  & 1 (0.023) & 1 (0.017) \\
%  bm & 1 (0.014) & 1.27   & 0.21  & 1 (0.004) & 0.67 & 1 (0.033) &  & 1 (0.054) & 1 (0.060) \\\midrule
%  GM & 1         & 1.80   & 0.67  & 1         & 1.17 & 1         &  & 1         & 1         \\
% \bottomrule
% \end{tabular}
% }

% The format DIA-V is a short name of the DIA-variant format. Empty cells (`-') are due to segmentation fault errors of the generated conversion code. 
% \resizebox{\textwidth}{!}{
% \begin{tabular}{c|ccc|ccc|cc|c|c}
% \toprule
% \multirow{2}{*}{\makecell{\textbf{Data}}} & \multicolumn{3}{c|}{\textbf{CSR -> CSC}} & \multicolumn{3}{c|}{\textbf{COO -> DIA}}  & \multicolumn{2}{c|}{\textbf{DCSR -> ELL}} &  \textbf{DCSC -> BCSR} & \textbf{CSB -> DIA-V} \\
% \cmidrule{2-11} 
%  & \IRName & \makecell{MLIR\\SparseTensor} & TACO & \makecell{\IRName\\w/ fusion} & \makecell{\IRName\\w/o fusion} & TACO & \IRName & TACO & \IRName & \IRName  \\\hline
%  wv & 1 (0.002) & 1.01   & 37.20 & 1 (0.104) & 0.78 & 0.86 & 1 (0.883) & & (0.019) & (0.065) \\
%  ee & 1 (0.000) & 2.58  & 11.17 & 1 (0.004) & 0.93 & 1.14 & 1 (0.020) & & (0.003) & (0.004) \\
%  nm & 1 (0.009) & 2.90   & 0.62  & 1 (0.004) & 3.05 & 1.95 & 1 (0.034) & & (0.038) & (0.030) \\
%  cm & 1 (0.003) & 1.65   & 0.32  & 1 (0.001) & 2.91 & 1.12 & 1 (0.009) & & (0.014) & (0.009) \\
%  ct & 1 (0.043) & 1.79   & 0.72  & 1 (0.018) & 3.11 & 1.88 & 1 (0.170) & & (0.151) & (0.169) \\
%  lp & 1 (0.672) & 0.98   & 0.56  & 1 (0.430) & 2.69 & 0.96 & 1 (4.103) & & (2.634) & (4.352) \\
%  tp & 1 (0.467) & 1.19   & 0.27  & 1 (0.148) & 5.02 & 0.93 & 1 (1.619) & & (2.335) & (5.584) \\
%  ts & 1 (0.534) & 0.85   & 0.31  & 1 (0.185) & 3.11 & 1.01 & 1 (4.768) & & (1.651) & (2.319) \\
%  ch & 1 (0.005) & 1.01   & 0.17  & 1 (0.001) & 5.27 & 0.98 & 1 (0.009) & & (0.017) & (0.012) \\
%  mj & 1 (0.033) & 1.25   & 0.27  & 1 (0.011) & 3.31 & 0.91 & 1 (0.082) & & (0.130) & (0.153) \\
%  sh & 1 (0.006) & 1.35   & 0.30  & 1 (0.002) & 3.05 & 0.84 & 1 (0.022) & & (0.023) & (0.017) \\
%  bm & 1 (0.014) & 1.27   & 0.21  & 1 (0.004) & 2.99 & 0.67 & 1 (0.033) & & (0.054) & (0.060) \\\midrule
%  GM & 1         & 1.80   & 0.67  & 1         & 2.32 & 1.17 & 1         & &         &         \\
% \bottomrule
% \end{tabular}
% }

% \begin{tabular}{c|ccc|c|c|ccc|c|c}
% \toprule
% \multirow{2}{*}{\makecell{\textbf{Data}}} & \multicolumn{3}{c|}{\textbf{CSR -> CSC}} & \textbf{COO -> BDIA} & \multirow{2}{*}{\makecell{\textbf{Data}}} & \multicolumn{3}{c|}{\textbf{COO -> DIA}}  & \multirow{2}{*}{\makecell{\textbf{Data}}} &  \textbf{COO -> BELL}  \\
% \cmidrule{2-4} \cmidrule{5-5} \cmidrule{7-9} \cmidrule{11-11} 
%  & \IRName & \makecell{MLIR\\SparseTensor} & TACO & \IRName & & \makecell{\IRName\\w/ fusion} & \makecell{\IRName\\w/o fusion} & TACO &  & \IRName  \\\hline
%  ge & 1(2.512) & 1.14(2.867) &  & (8.946) & wv & 1(0.104) & 0.78(0.081) & 0.81(0.084) & c8 & (0.118) \\
%  ss & 1(0.863) & 1.24(1.073) &  & (1.203) & ee & 1(0.004) & 0.93(0.004) & 1.40(0.006) & ee & (0.001) \\
%  ra & 1(0.573) & 1.08(0.617) &  & (0.733) & nm & 1(0.004) & 3.05(0.013) & 2.07(0.009) & nm & (0.060) \\
%  mc & 1(0.393) & 1.18(0.464) &  & ()      & cm & 1(0.001) & 2.91(0.003) & 1.09(0.001) & h1 & (0.074) \\
%  vs & 1(1.137) & 1.11(1.262) &  & (0.660) & ct & 1(0.018) & 3.11(0.055) & 1.91(0.034) & b9 & (0.089) \\
%  lp & 1(0.619) & 1.09(0.674) &  & (2.082) & lp & 1(0.430) & 2.69(1.156) & 0.89(0.382) & cr & (0.008) \\
%  tp & 1(0.487) & 1.19(0.582) &  & (2.090) & tp & 1(0.148) & 5.02(0.744) & 0.82(0.122) & tf-0.6 & (0.339) \\
%  ts & 1(0.562) & 0.83(0.466) &  & (1.359) & ts & 1(0.185) & 3.11(0.576) & 0.89(0.165) & tf-0.7 & (0.274) \\
% \bottomrule
% \end{tabular}

% \resizebox{0.48\textwidth}{!}{
% \begin{tabular}{c|ccc|c}
% \toprule
% \multirow{2}{*}{\textbf{Data}} & \multicolumn{3}{c|}{\textbf{CSR -> CSC}} & \textbf{COO -> BELL} \\
% \cmidrule{2-4} \cmidrule{5-5}  
%  & \IRName & \makecell{MLIR\\{SparseTensor}} & {TACO} & \IRName \\\hline
% % wv &  &  &  & 1(0.104) & 0.78(0.081) & 0.81(0.084) &  &  \\
% % ee &  &  &  & 1(0.004) & 0.93(0.004) & 1.40(0.006) &  &  \\
% % nm &  &  &  & 1(0.004) & 3.05(0.013) & 2.07(0.009) &  &  \\
% % cm &  &  &  & 1(0.001) & 2.91(0.003) & 1.09(0.001) &  &  \\
% % ct &  &  &  & 1(0.018) & 3.11(0.055) & 1.91(0.034) &  &  \\
% % lp &  &  &  & 1(0.430) & 2.69(1.156) & 0.89(0.382) &  &  \\
% % tp &  &  &  & 1(0.148) & 5.02(0.744) & 0.82(0.122) &  &  \\
% % ts &  &  &  & 1(0.185) & 3.11(0.576) & 0.89(0.165) &  &  \\
% % \cline{2-3}
% %                                              & \lstinline|relayout(lv)| & Rearrange the storage of subtensors specified by level \lstinline|lv| into specific memory spaces\\
% \bottomrule
% \end{tabular}
% }
% \resizebox{0.32\textwidth}{!}{
% \begin{tabular}{c|ccc}
% \toprule
% \multirow{2}{*}{\textbf{Data}} & \multicolumn{3}{c}{\textbf{COO -> DIA}} \\
% \cmidrule{2-4} 
%  & \IRName & \makecell{\IRName\\w/o fusion} & TACO \\\hline

% % \cline{2-3}
% %                                              & \lstinline|relayout(lv)| & Rearrange the storage of subtensors specified by level \lstinline|lv| into specific memory spaces\\
% \bottomrule
% \end{tabular}
% }
% \resizebox{0.19\textwidth}{!}{
% \begin{tabular}{c|c}
% \toprule
% \multirow{2}{*}{\textbf{Data}} & \multicolumn{1}{c}{\textbf{COO -> BDIA}} \\
% \cmidrule{2-2} 
%  & \IRName \\\hline

% % \cline{2-3}
% %                                              & \lstinline|relayout(lv)| & Rearrange the storage of subtensors specified by level \lstinline|lv| into specific memory spaces\\
% \bottomrule
% \end{tabular}
% }

% \resizebox{0.69\textwidth}{!}{
% \begin{tabular}{c|ccc|ccc|c|c}
% \toprule
% \multirow{2}{*}{\lstinline{DS}} & \multicolumn{3}{c|}{\lstinline{CSR -> CSC}} & \multicolumn{3}{c|}{\lstinline{COO -> DIA}} & \lstinline{COO -> BDIA} & \lstinline{COO -> BELL} \\
% \cmidrule{2-4} \cmidrule{5-7} \cmidrule{8-8} \cmidrule{9-9} 
%  & \IRName & \makecell{MLIR\\SparseTensor} & TACO & \IRName & \makecell{\IRName\\w/o fusion} & TACO & \IRName & \IRName \\\hline
% wv &  &  &  & 1(0.104) & 0.78(0.081) & 0.81(0.084) &  &  \\
% ee &  &  &  & 1(0.004) & 0.93(0.004) & 1.40(0.006) &  &  \\
% nm &  &  &  & 1(0.004) & 3.05(0.013) & 2.07(0.009) &  &  \\
% cm &  &  &  & 1(0.001) & 2.91(0.003) & 1.09(0.001) &  &  \\
% ct &  &  &  & 1(0.018) & 3.11(0.055) & 1.91(0.034) &  &  \\
% lp &  &  &  & 1(0.430) & 2.69(1.156) & 0.89(0.382) &  &  \\
% tp &  &  &  & 1(0.148) & 5.02(0.744) & 0.82(0.122) &  &  \\
% ts &  &  &  & 1(0.185) & 3.11(0.576) & 0.89(0.165) &  &  \\
% % \cline{2-3}
% %                                              & \lstinline|relayout(lv)| & Rearrange the storage of subtensors specified by level \lstinline|lv| into specific memory spaces\\
% \bottomrule
% \end{tabular}
% }

% \multirow{2}{*}{\lstinline{Data}} & \multicolumn{3}{c|}{\lstinline{CSR -> CSC}} & \lstinline{COO -> BELL} \\
% \cmidrule{2-4} \cmidrule{5-5}  
%  & \lstinline{UniSparse} & \makecell{\lstinline{MLIR}\\\lstinline{SparseTensor}} & \lstinline{TACO} & \lstinline{UniSparse} \\\hline
 

==> figs-tabs/tab-pagerank.tex <==
\begin{table}[ht]%[tb!]
\centering
% \vspace{-5pt}
\caption{
\newrev{}}
\footnotesize
\setlength\tabcolsep{5pt} % Reduce the white space margins in each cell
\lstset{%
tabsize=2,
columns=fullflexible,
basicstyle=\ttfamily\scriptsize,
breaklines=true,
breakatwhitespace,
escapeinside={(*}{*)},
alsoletter={\., \_},
morekeywords={tile\_division, tile\_union, enumerate, reorder, schedule, move\_lv, trim, fill, merge, split, vectorize, devectorize, pad, pack, partition}
}
\resizebox{0.7\textwidth}{!}{\newtablerev
\begin{tabular}{c|c|c|c|c|c}
\toprule
\multirow{2}{*}{\makecell{\thead{\textbf{Data}}}} & \multirow{2}{*}{\makecell{\thead{\textbf{Iterations}}}} & \multicolumn{3}{c|}{\thead{\textbf{BDIA/CSR in \IRName}}} & \multirow{2}{*}{\makecell{\thead{\textbf{CSR in MKL}}}} \\
\cmidrule{3-5} 
    &   & \makecell{Format Conversion} & Kernel Execution & Total &   \\\midrule
    &   &   &   &   &   \\
    &   &   &   &   &   \\
    &   &   &   &   &   \\
    &   &   &   &   &   \\\midrule
 Geomean &   &   &   &   &   \\
\bottomrule
\end{tabular}
}
\label{tab:pagerank}
\end{table}

